Approximate Similarity Search Under Edit Distance Using Locality-Sensitive Hashing

Edit distance similarity search, also called approximate pattern matching, is a fundamental problem with widespread database applications. The goal of the problem is to preprocess $n$ strings of length $d$, to quickly answer queries $q$ of the form: if there is a database string within edit distance $r$ of $q$, return a database string within edit distance $cr$ of $q$. Previous approaches to this problem either rely on very large (superconstant) approximation ratios $c$, or very small search radii $r$. Outside of a narrow parameter range, these solutions are not competitive with trivially searching through all $n$ strings. In this work give a simple and easy-to-implement hash function that can quickly answer queries for a wide range of parameters. Specifically, our strategy can answer queries in time $\tilde{O}(d3^rn^{1/c})$. The best known practical results require $c \gg r$ to achieve any correctness guarantee; meanwhile, the best known theoretical results are very involved and difficult to implement, and require query time at least $24^r$. Our results significantly broaden the range of parameters for which we can achieve nontrivial bounds, while retaining the practicality of a locality-sensitive hash function. We also show how to apply our ideas to the closely-related Approximate Nearest Neighbor problem for edit distance, obtaining similar time bounds.

==> ack.tex <==
\section{Acknowledgements}
\seclabel{ack}


==> conclusion.tex <==
\section{Conclusion}
\seclabel{conclusion}

1. Random strings
2. Other costs
3. Getting around the lower bound--can knowledge of the data help?
4. What are the common cases for edit distance? What bounds can we give?


==> lower.tex <==
\section{Lower Bound}

Ideally, we would like to obtain an LSH that removes the $3^r$ (TODO) term, obtaining a running time of $n^{\rho}$ where $\rho$ is a function of $c$ alone.  In this section, we rule out this possibility by showing that TODO.

Our lower bound applies to ``LSH-like'' functions.  In particular, we use the \defn{list of points} model of Andoni et al.  Briefly, in this model, we consider algorithms that partition the space probabilistically into hash buckets.  On a query, the algorithm scans through a subset of these buckets---this subset is a function of the query alone, and may not adapt dynamically based on what is seen in previous buckets.  The algorithm must guarantee that any point within distance $r$ of the query is in one of these buckets with constant probability.  The cost is the total number of points in all buckets inspected, plus the number of inspected buckets.  See \cite[Definition 1.5]{AndoniLaRa17} for a formal definition.

TODO: discussion here of how this is different from the embedding lower bounds (those lower bounds are easy cases for nearest neighbor search), and what it has in common (if you're doing well with a small number of replacements you are close to a function that looks at very few coordinates; but those functions do very poorly with alignments). 

%Our bound uses many of the same techniques as the lower bound for embedding edit distance of Khot and Naor~\cite{TODO}.  
We begin by showing that any efficient algorithm in the list of points model implies the existence of a Boolean function that satisfies certain properties.
%used in the embedding lower bound of Khot and Naor.  
%We subsequently show using the techniques of~\cite{} that this function does not exist.
We then use Boolean function analysis to show that this function cannot exist, following the same high-level strategy as the embedding lower bound of Khot and Naor~\cite{KhotNaor06}.  (This lower bound was improved in later work, but their techniques seem more amenable to our hard distribution.)

\subsection{Preliminaries}

We construct our hard distribution using an alphabet of size $2$.  In particular, we will treat all strings as elements of $\field_2^d$; this will let us describe our hard distribution more simply---for example, it allows us to perturb a string by adding a noise vector.   

Let $\mu$ be the uniform random distribution over $\field_2^d$; a given $x\in\field_2^d$ occurs with probability $1/2^d$.  Let $\mu_{\epsilon}$ be TODO.  

We (in part) use Fourier analysis to prove our lower bound.  This part of the analysis follows the ideas of Khot and Noar fairly closely~\cite{KhotNaor06}; their manuscript has a good background exposition of these techniques. Further details can be found in~\cite{ODonnell14}. 

\subsection{Proof of TODO}

\begin{lemma}
  \lemlabel{lshtobool}
  If there is an algorithm in the list-of-points model with running time $O(\min\{2^{\sqrt{r}}, \sqrt{n}\})$, then there exists a Boolean function $f:\{0,1\}^d\rightarrow\{0,1\}$ such that
\end{lemma}
\begin{proof}
\end{proof}

The dataset for our lower bound will consist of $n$ points from the following distribution.
\begin{definition}
\end{definition}

%We show that these points are far points (have distance $\geq cr$ from the query $q$) with high probability.  This means that this distribution is suitable for use in \lemref{TODO}.  This bound is fairly rough and ultimately follows known strategies, like~\cite[Lemma 8]{KhotNaor06}.
%
%\begin{lemma}
%  \lemlabel{randompointsfar}
%If $d > 2\log n$, 
%  \[
%    \Pr_{x,y\sim \mu_F} (\ED(x,y) \geq d/20 - \sqrt{r}) \geq 1 - 1/n
%  \]
%\end{lemma}
%
%\begin{proof}
%Hopefully the string definition we used in the prelim will make it clear that 
%  \[
%     |y\in F_2^d \ED(x,y) = r| \leq 2^r\binom{2d}{r}
%  \]
%Thus,
%  \begin{align*}
%    \Pr_{x,y\sim\mu} (\ED(x,y)\geq d/20) &\geq 1 - \frac{1}{2^d} \sum_{r\leq d/10} 2^r\binom{2d}{r}\\
%    &\geq 1 - \frac{1}{2^d} \sum_{r\leq d/20} 2^r \left(\frac{2de}{r}\right)^r\\
%    &\geq 1 - \frac{1}{2^d} \sum_{r\leq d/20} \left(\frac{4de}{r}\right)^r\\
%    &\geq 1 - \frac{1}{2^d} \sum_{r\leq d/20} \left(\frac{4de}{r}\right)^r\\
%    &\geq 1 - \frac{1}{2^d} (80e)^{d/20 + 1}\\
%    &\geq 1 - 1/2^{d/2}
%  \end{align*}
%
%  The fact that we're keeping some digits the same will affect the denominator of the term before the sum.  But if the number of digits we're keeping the same is $< d/2$ we get the same bound.  (Maybe need to change to $d/4$.) 
%\end{proof}

%We ignore any points violating \lemref{randompointsfar} for the remainder of our analysis.

The following lemma shows that any function which is unlikely to change value when permuting the digits and adding an $\epsilon$-weight vector must have Fourrier coefficients satisfying a certain useful property.  This proof is almost exactly the first half of the proof of Lemma 7 in~\cite{KhotNaor06}.

\begin{lemma}
  For every $f: \{0,1\}^d\rightarrow\{-1,1\}$ and every permutation $\pi$, 
  %if 
  %\[
  %  \int_{\{0,1\}^d\times \{0,1\}^d} |f(x) - f(\pi(x) + y)| d\mu(x) d\mu_{\epsilon}(y) \geq 1/2^r
  %  \]
  %then
  %\[
  %  \sum_{A\subseteq\{1,\ldots,d\}} (1 - \epsilon)^{|A|}\hat{f}(A)^2 \geq 1 - 1/2^r.
  %  \]
  \[
    \sum_{A\subseteq\{1,\ldots,d\}} (1 - \epsilon)^{|A|}\hat{f}(A)^2 \geq  1 - \int_{\{0,1\}^d\times \{0,1\}^d} |f(x) - f(\pi(x) + y)| d\mu(x) d\mu_{\epsilon}(y) 
    \]
\end{lemma}

\begin{proof}
  Define the Walsh function
  \[
    W_A(x) = (-1)^{\sum_{j\in A} x_j}.
  \]
Thus, the Fourier expansion of $f$ can be written as $f = \sum_A \hat{f}(A) W_A$.

  The proof proceeds in the following steps, which we explain below.
  \begin{align}
    &\int_{\field_2^d\times\field_2^d} |f(x) - f(\pi(x) + y)| d\mu(x) d\mu_{\epsilon}(y) \label{step1}\\
    &\qquad\qquad= 1 - \int_{\field_2^d\times\field_2^d} f(x)f(\pi(x) + y) d\mu(x) d\mu_{\epsilon}(y)\label{step2}\\
    &\qquad\qquad= 1 - \int_{\field_2^d\times\field_2^d} \left( \sum_{A,B\subseteq\{1,\ldots,d\}} \hat{f}(A)\hat{f}(B) W_A(x)W_B(\pi(x) + y)\right) d\mu(x) d\mu_{\epsilon}(y)\label{step3}\\
    &\qquad\qquad= 1 - \int_{\field_2^d\times\field_2^d} \left( \sum_{A,B\subseteq\{1,\ldots,d\}} \hat{f}(A)\hat{f}(B) W_A(x)W_{\pi^{-1}(B)}(x)W_B(y)\right) d\mu(x) d\mu_{\epsilon}(y)\label{step4}\\
    &\qquad\qquad= 1 - \sum_{A\subseteq\{1,\ldots,d\}} (1 - 2\epsilon)^{|A|} \hat{f}(A)\hat{f}(\pi(A))\label{step5}\\
    &\qquad\qquad\geq 1 - \sum_{A\subseteq\{1,\ldots,d\}} (1 - 2\epsilon)^{|A|} \hat{f}(A)^2\label{step6}
  \end{align}

  \stepheading{step1}{step2} Since $f(x)\in\{-1,1\}$ for all $x$ (and all $y$), $|f(x) - f(y)| = 1 - f(x)f(y)$ for all $x,y$.  

  \stepheading{step2}{step4} By definition of $W$.

  \stepheading{step4}{step5} Take a dimension $i\in (B\setminus\pi(A))\cup(\pi(A)\setminus B)$.  When we integrate over all $x\in\field_2^d$, $x_i = 1$ and $x_i = -1$ an equal number of times; thus, $\int_{\field_2^d} W_A W_{\pi^{-1}(B)} d\mu = 0$ when $B\neq \pi(A)$.

  \stepheading{step5}{step6} Follows directly from the Cauchy-Schwartz inequality.
\end{proof}

The following theorem, originally due to Bourgain~\cite{Bourgain02}, was reproven with the following parameters in \cite{KhotNaor06}.  

\begin{theorem}[Bourgain's noise sensitivity theorem~\cite{KhotNaor06,Bourgain02}]
  Fix $\epsilon,\delta\in(0,1/10)$ and a Boolean function $f:F^d_2\rightarrow\{-1,1\}$
  Assume that 
  \[
    \sum_{A\subseteq\{1,\ldots,d\}} (1-\epsilon)^{|A|}\hat{f}(A)^2 \geq 1 - \delta
    \]
  Then there is a universal constant $C$ where for every $\beta > 0$ there exists a function $g: \field_2^d\rightarrow\reals$ which depends on at most $1/\epsilon\beta$ coordinates, such that
  \[
    \int_{\field_2^d} (f(x) - g(x))^2 \leq 2^{C\sqrt{\log(1/\delta)\log\log(1/\epsilon)}}\left(\frac{\delta}{\sqrt{\epsilon}} + 4^{1/\epsilon}\sqrt{\beta}\right).
    \]
\end{theorem}

The following lemma is the key indistinguishability lemma in our lower bound.  
A function $g$ which only looks at a subset of dimensions will only be able to ``catch'' our misalignment if TODO.
%If a function $g$ looks only at dimensions that are permuted the same way in the far distribution as they are for the close point, $g$ cannot distinguish close points from far points.

We call a permutation $\pi_2$ \defn{$I$-invariant} to a permutation $\pi_1$ for a set $I\subseteq \{1,\ldots,d\}$ if for all $i\in I$, if $\pi_1(i)\in I$, then $\pi_2(i) = \pi_1(i)$.  

\begin{lemma}
  Consider a function $g: \field_2^d \rightarrow\reals$ that depends on at most $t$ coordinates $I = i_1,\ldots,i_t$. 
  %Let $\pi_1$ be an arbitrary permutation, and let $\pi_2$ be a permutation such that for all $i_j$ such that $i_j\in I$ and $\pi_1(i_j)\in I$, $\pi_2(i_j) = \pi_1(i_j)$.  
  
  %For a given permutation $\pi$, consider the maximal subset of these coordinates $J_{\pi}\subseteq I$ such that for all $j\in J_{\pi}$, either $\pi(j) \in I$ or $\pi^{-1}(j)\in I$.

  %Then for two permutations $\pi_1$ and $\pi_2$, if $J_{\pi_1} = J_{\pi_2}$, then
  Then for any permutations $\pi_1,\pi_2$ such that $\pi_2$ is $I$-invariant to $\pi_1$,
  \[
    \int_{\field_2^d\times\field_2^d} |g(x) - g(\pi_1(x) + y)|d\mu(x)d\mu_{\epsilon}(y)
    = \int_{\field_2^d\times\field_2^d} |g(x) - g(\pi_2(x) + y)|d\mu(x)d\mu^{\pi_2}(y)
    \]
\end{lemma}
\begin{proof}
  For each $x$, let $x^I$ be a $t$-dimensional vector such that for $k = 1,\ldots, t$, $x^I_k = x_{i_k}$.
\end{proof}

Need a distribution of close permutations and a distribution of far permutations. 

\begin{lemma}
  For any set $I$ of size $t \leq TODO$, 
  \[
    \Pr_{\substack{\pi_1\sim S_{\textnormal{close}} \\ \pi_2\sim S_{\textnormal{far}}}} \left(\pi_2 \textnormal{ is $I$-invariant to } \pi_1\right) \geq \frac{1}{\left(\sqrt{r}\right)^{\sqrt{r}}}
  \]
\end{lemma}

Putting these together, we obtain the following lemma, which contradicts the requirements of \lemref{lshtobool}.

\begin{lemma}
  If $f$ satisfies
  \[
    \int_{\{0,1\}^d\times \{0,1\}^d} |f(x) - f(\pi(x) + y)| d\mu(x) d\mu_{\epsilon}(y) \geq 1/2^r
    \]
  then
  (something like: the average far(ish) point which is the same in $1/\sqrt{r}$ coordinates and then has a bunch of shifts collides with probability at least $1/\sqrt{n}$.)
\end{lemma} 


==> old.tex <==

%%%%%% Unnecessary lower bound on probability

\begin{lemma}
  \lemlabel{probinduceslower}
  For any $\$$-terminal strings $x$ and $y$, let $T$ be a transformation of length $t$ 
  %such that $T(x,y) = y$ and $T$ is prefix-free for $x$ and $y$.  
  that solves $x$ and $y$.  
  Then
  \[
    \Pr_\rho[T = \calT(x,y,\rho)] \geq p^t/4.
  \]
  %Let $x$ and $y$ be $\$$-terminal strings, and 
  %let $T$ be a transformation of length $t$ such that $T(x,y) = y$.  Then
  %\[
  %  \Pr_\rho[T = \calT(x,y,\rho)] \geq p^t.
  %\]
\end{lemma}
\begin{proof}
  We begin by defining a sequence of pairs.  Let $g(x,y,\rho)$ be an alive grid walk such that deleting $\loo{}$ and \match{} from $g$ results in $T$; this walk must exist by \todo{needs to depend on solving}.  We begin by listing all vertex pairs in order traversed by the corresponding grid walk: $\big((i(x,0,\rho),i(y,0,\rho)), (i(x,1,\rho),i(y,1,\rho)), \ldots, (i(x,|g(x,y,\rho)|,\rho),i(y,|g(x,y,\rho)|,\rho)\big)$.  We then delete all duplicates from this sequence to obtain a sequence $\big((i_1,j_1),(i_2,j_2),\ldots\big)$.  Note that the resulting sequence is the same regardless of which grid walk we started with because each new vertex traversed by the grid walk corresponds to an \ins{}, \del{}, or \rep{} that corresponds to a vertex in $T$, or a \match{} which is taken for every $\rho$.  We call this (unique) sequence the \defn{node walk} of $T$, and we say that $g(x,y,\rho)$ \defn{traverses} this node walk. 

  %For a given node walk, let $m_k$ be the number of aligned characters between $(i_k,j_k)$ and $(i_{k+1},j_{k+1})$.  Thus, $m_k$ is the largest number such that \todo{fill out definition once off by one is figured out, and then define how grid walks traverse sequences}

  For a given node walk $((i_1,j_1),(i_2,j_2),\ldots)$ and a given $\ell$, let $m_{\ell}$ be the number of $(i_k,j_k)$ with $k < \ell$ and $x_{i_k} \neq y_{i_k}$.  

  Note that an operation is added to $T$ exactly once each time the grid walk traverses a non-matching node; thus if the node walk of $T$ has length $L$, then $m_L = |T|$.  Furthermore, each time an operation is added to the node walk, either $i(x,k,\rho)$ or $i(y,k,\rho)$ increases; thus $L \leq |x| + |y| \leq 2d$.

  We lower bound $\Pr_{\rho}[T = \calT(x,y,\rho)]$ by only considering grid walks that have at most $(\log_{1/p_a} 2d)$ \loo{} operations between any two consecutive non-\loo{} operations.  In particular, all grid walks satisfying this condition have length at most $d\log_{1/p_a} 2d < (3d\log d)/(1-p_a)$. 

  The remainder of this proof shows the following claim by induction on $\ell$.
  \begin{claim}
    \claimlabel{inductivepaths}
    Let $T$ have grid walk $\big((i_1,j_1),\ldots\big)$.  Then the probability that $g(x,y,\rho)$ traverses nodes $(i_1,j_1), (i_2,j_2),\ldots (i_\ell,j_\ell)$ such that $g(x,y,\rho)$ has at most $(\log_{1/p_a} 2d)$ \loo{} operations between any two consecutive non-\loo{} operations is at least $p^{m_{\ell}}(1-1/2d)^\ell$.
  \end{claim}
  \begin{proof}
    If $k = 0$, the claim is satisfied because all grid walks begin at $(0,0)$.

        Let $E_{\rho,\ell}$ be the event that $g(x,y,\rho)$ traverses $(i_1,j_1),\ldots, (i_\ell,j_\ell)$, and that $g(x,y,\rho)$ has at most $(\log_{1/p_a} 2d)$ \loo{} operations between any two successive non-\loo{} operations. 
Let $k(\ell,\rho)$ be the integer satisfying $i(x,k(\ell,\rho),{\rho}) = i_{\ell-1}$ and $i(y,k(\ell,\rho),{\rho}) = j_{\ell-1}$.  In other words, the grid walk under ${\rho}$ takes $k(\ell,\rho)$ grid walk steps before encountering $\ell$ \ins{}, \del{}, or \rep{} operations.

    Assume inductively that $\Pr[E_{\rho,\ell - 1}] \geq p^{m_{\ell-1}} (1 - 1/2d)^{\ell - 1}$.
    %the probability that $g(x,y,\rho)$ traverses $(i_1,j_1),\ldots (i_{\ell-1},j_{\ell-1})$ is at least $p^{\ell-1}(1 - p^x)^{m'}$, where $m' = \sum_{\ell' < \ell-1} m_{\ell'}$.  

    %\todo{move/remove} Consider a  $\hat{\rho}$ such that $g(x,y,\hat{\rho})$ traverses $((i_1,j_1),\ldots, (i_{\ell-1},j_{\ell-1})$.  


        %The remainder of this proof bounds 
      Event $E_{\rho,\ell-1}$ must always occur if $E_{\rho,\ell}$ occurs; so $\Pr[E_{\rho,\ell}] =  \Pr[E_{\rho,\ell - 1}] \cdot \Pr[E_{\rho,\ell} ~|~ E_{\rho,\ell -1 }]$.  
        Thus, the remainder of this proof uses  $\Pr[E_{\rho,\ell} ~|~ E_{\rho,\ell-1}]$ to bound $\Pr[E_{\rho,\ell}]$.  
        %\[ \Pr[g(x,y,\hat{\rho}) \text{ traverses } (i_\ell,j_\ell) ~|~ g(x,y,\hat{\rho}) \text{ traverses } (i_1,j_1),\ldots (i_{\ell-1},j_{\ell -1})].  \] 
    We split into four cases based on $(i_\ell,j_\ell)$.

    \noindent
      \textbf{Case 1 ($x_{i_{\ell-1}} = y_{j_{\ell-1}}$):} in this case, both hashes write the same character to $s$: 
      %$\rho(x_{i_{\ell-1}},k(\ell,\rho)) = \rho(y_{j_{\ell-1}},k(\ell,\rho))$ for all $\rho$ and $\ell$.  
      $\tau_{k(\ell,\rho)}(x,\rho) = \tau_{k(\ell,\rho)}(y,\rho)$ for all $\rho$.  
      Thus, the probability that $g_{k(\ell,\rho)}(x,y,{\rho}) = \loo{}$ is $p_a$, and the probability that  $g_{k(\ell,\rho)}(x,y,{\rho}) = \match{}$ is $1 - p_a$.  If $g_{k(\ell,\rho)}(x,y,\rho) = \loo{}$, then the probability that $g_{k(\ell,\rho)+1}(x,y,\rho) = \loo$ is again $p_a$, and so on.  Thus the probability that $g(x,y,{\rho})$ has at most $\log_{1/p_a} 2d$ consecutive \loo{} operations before traversing $(i_\ell,j_\ell)$ is at least $1 - p_a^{(\log_{1/p_a} 2d)} = 1 - 1/2d$.  Thus we have $\Pr[E_{\rho,\ell} ~|~ E_{\rho, \ell-1} ] = (1 - 1/2d)$.  Furthermore, $m_{\ell} = m_{\ell - 1}$.  Substituting, 
      %Events $E_{\rho,\ell}$ and $E_{\rho,\ell - 1}$ are independent by definition of $\rho$, \todo{does this use Bayes' rule?}
      %From the inductive assumption, $\Pr[E_{\rho,\ell-1}]\geq p^{\ell - m' - 1}(1- p_a^x)^{m'}$; thus 
      \[
        \Pr[E_{\rho,\ell}] \geq p^{m_{\ell - 1}}(1 - 1/2d)^{\ell-1}(1 - 1/2d) = p^{m_{\ell}}(1 - 1/2d)^\ell
      \]
      %since $\sum_{\ell' < \ell} m_{\ell'} = 1 + \sum_{\ell' < \ell - 1} m_{\ell'}$.
      %since $m_{\ell} = m_{\ell - 1}$. 

    \noindent
      \textbf{Case 2 ($x_{i_{\ell - 1}}\neq y_{j_{\ell-1}}$, $i_\ell = i_{\ell-1}$, and $j_\ell = j_{\ell-1} + 1$):}
        From the definition of a grid walk, $g(x,y,{\rho})$ traverses $(i_\ell,j_\ell)$ only if, for some $X'$, $g_{k'}(x,y,{\rho}) = \loo{}$ for all $k(\ell,\rho) \leq k' < k(\ell,\rho) + X'$, and $g_{k(\ell,\rho) + X'}(x,y,{\rho}) = \del{}$.  
        By \lemref{gridwalkprobs}, this occurs with probability $p_a^{2X'} p_a(1-p_a)p_r$ conditioned on $E_{\rho,\ell-1}$.  
        %(we know that $\Pr_{\rho}[E_{k}] > 0$ by the inductive hypothesis; furthermore, the bound \todo{loops imply shortish walks}).  
        Summing over all $X'$, we obtain 
        \begin{align*}
          \Pr[E_{\rho,\ell} ~|~ E_{\rho,\ell-1} ] &\geq \sum_{X' < \log_{1/p_a} 2d} p_a^{2X'} p_a(1-p_a) p_r\\
          & = p_a (1-p_a) p_r \frac{1 - p_a^{2\log_{1/p_a} 2d}}{1 - p_a^2}\\
          &= p(1 - 1/4d^2)
        \end{align*}
        Where the last step follows from $p_r = p_a/(1-p_a)$ and $p_a^2/(1- p_a^2) = p$.  Since $m_{\ell} = m_{\ell - 1} + 1$, 
        %As in Case 1 we obtain 
        \[
          \Pr[E_{\rho,\ell}] = p^{m_{\ell - 1} }(1 - 1/2d)^{\ell - 1}p(1 - 1/4d^2) \geq p^{m_{\ell}}(1-1/2d)^\ell.
        \]
        %where the last step is due to \todo{$\ell$ and $m$} and $1 - p_a^{2X} \geq 1 - p_a^X$. 


    \noindent
      \textbf{Case 3 ($x_{i_{\ell - 1}}\neq y_{j_{\ell-1}}$, $i_k = i_{k} + 1$, and $j_k = j_{k-1}$):} The argument corresponds exactly to Case 2 with \ins{} instead of \del{}.

    \noindent
      \textbf{Case 4 ($x_{i_{\ell - 1}}\neq y_{j_{\ell-1}}$, $i_k = i_{k} + 1$, and $j_k = j_{k-1} + 1$):} 
        From the definition of a grid walk, $g(x,y,{\rho})$ traverses $(i_\ell,j_\ell)$ only if, for some $X'$, $g_{k'}(x,y,{\rho}) = \loo{}$ for all $k(\ell,\rho) \leq k' < k(\ell,\rho) + X'$, and $g_{k(\ell,\rho) + X'}(x,y,{\rho}) = \rep{}$.  
        By \lemref{gridwalkprobs}, this occurs with probability $p_a^{2X'} (1-p_a)^2p_r^2$ conditioned on $E_{\rho,\ell-1}$.  
        %(we know that $\Pr_{\rho}[E_{k}] > 0$ by the inductive hypothesis; furthermore, the bound \todo{loops imply shortish walks}).  
        Summing over all $X'$ as in Case 2, we obtain 
        \begin{align*}
          \Pr[E_{\rho,\ell} ~|~ E_{\rho,\ell-1} ] &\geq \sum_{X' < \log_{1/p_a} 2d} p_a^{2X'} (1-p_a)^2 p_r^2\\
          &= p(1 - 1/4d^2).
        \end{align*}
        %Where the last step follows from $p_r = p_a/(1-p_a)$ and $p_a^2/(1- p_a^2) = p$.  
        Since $m_{\ell} = m_{\ell - 1} + 1$, 
        %As in Case 1 we obtain 
        \[
          \Pr[E_{\rho,\ell}] = p^{m_{\ell - 1} }(1 - 1/2d)^{\ell - 1}p(1 - 1/4d^2) \geq p^{m_{\ell}}(1-1/2d)^\ell.
        \]
  \end{proof}
  Let $L$ be the length of the node walk corresponding to $T$.  Invoking \claimref{inductivepaths} with $\ell = L$, and recalling that $m_L = t$, $L \leq 2d$, and $d \geq 2$ we can upper bound
  \[
    \Pr_{\rho}[T = \calT(x,y,\rho)] \geq p^t(1 - 1/2d)^L \geq p^t(1-1/2d)^{2d} \geq p^t/4.
  \]
  %We have that $t = \ell - m$ by definition.  Meanwhile, since \todo{fill in for $X$}.  Thus, $\Pr[T = \calT(x,y,\rho)] \geq p^t/2$. 
  %Setting $k = r$, and noting that $2d - r \geq \sum m_k \geq d - r$, we obtain the lemma.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLDER

Each underlying function, given $x$ and $y$,  $\defn{induces}$ a transformation using a process defined in \defref{inducedtransformations}. \defref{inducedtransformations} and \lemref{transformationcorrect} form the main idea behind our hash: $x$ and $y$ have a hash collision if and only if the induced transformation, when applied to $x$, successfully transforms it into $y$.  


\begin{definition}
  \deflabel{inducedtransformations}
  Consider two strings $x$ and $y$ and an underlying function $\rho$.  
  The following process determines the transformation $T$ induced by $x$, $y$, and $\rho$ if it exists.
  %Then if $x$, $y$, and $\rho$ induce an alignment $T$, it is defined as follows.
  %tracing the construction of $s_$ step by step 
  %recursively as follows 
  %starting with the empty string $T = \Lambda$.   
  
  Assume $|h_\rho(x)| = |h_\rho(y)|$; otherwise we say that $x$, $y$, and $\rho$ do not induce a transformation.
  We use $k$ to index the hashes $h_\rho(x)$ and $h_{\rho}(y)$.  Let $i(x,k,\rho)$ be the index of $x$ (i.e. the value of $i$) when the $k$th character of $h_\rho(x)$ is written; similarly, let $i(y,k,\rho)$ be the index of $y$ when the $k$th character of $h_{\rho}(y)$ is written.  
  
  %If $|h_\rho(x)| \neq |h_\rho(y)|$, then we say that $x$, $y$, and $\rho$ do not induce an alignment. 

  %We use $i$ as the index of $x$ when building $h(x)$, and $j$ as the index of $y$.  We begin with $i = j = 0$; $i$ and $j$ are incremented when $h(x)$ and $h(y)$ increment their respective indices.

  %\noindent
  %  If $x_i = y_j$: 
  %\begin{itemize}[topsep=0pt,noitemsep]
  %  \item  we add nothing to $T$.  Both hashes have $0$ or more hash-inserts, followed by a hash-replace or a hash-match which increments both $i$ and $j$. 
  %\end{itemize}
  %Otherwise, $x_i \neq y_j$, and: 
  We iterate through each position of $h_\rho(x)$ and $h_\rho(y)$, appending operations to $T$ one at a time.  Let $i = i(x,k,\rho)$ be the index of $x$ when the $k$th hash character is written, and $j = i(y,k,\rho)$ be the index of $y$ when the $k$th hash character is written.  

  \noindent
  If $x_i \neq y_j$, then: 
  \begin{itemize}[topsep=0pt,noitemsep]
    \item if $x_i$ has a hash-replace and $y_j$ has a hash-replace, we  append a ``replace'' to $T$. 
    \item If $x_i$ has a hash-replace and $y_j$ has a hash-insert,  we append a ``delete'' to $T$.
    \item If $x_i$ has a hash-insert and $y_j$ has a hash-replace,  we append an ``insert'' to $T$.
    \item If $x_i$ and $y_j$ both have a hash-insert, we do not add any operation to $T$.
    \item If $x_i$ or $y_j$ have a hash-match, then $x$, $y$, and $\rho$ do not induce a transformation.
\end{itemize}
If $x_i = y_j$, we do not add any operation to $T$.  
  %If none of the above cases applies, we do not add any operation to $T$. 
\end{definition}

%The above definition can lead to a $T$ that seems incomplete---for example, it may be that the process of constructing $T$ terminates because there are no further characters in $h_\rho(x)$, while there are many more in $h_\rho(y)$.  These cases correspond to $\rho$ where $h_\rho(x)\neq h_\rho(y)$.  

%TODO: the remaining discussion is dumb.  Just have a lemma saying that in all other cases the hashes are not equal---if $h_{\rho}(x) = h_{\rho}(y)$, then there is an induced transformation $T$ such that $T(x) = y$.  Also make sure that when the hash "dies" (as opposed to just not adding anything and trying again) is clear.
%
%Note that the remaining cases were intentionally excluded from the above definition.  If $x_i$ and $y_j$ both have a hash-insert, $i$ and $j$ do not increment; the hash makes no forward progress and we try again.
%If $x_i$ or $y_j$ has a hash-match (and $x_i \neq y_j$), they write different characters, and the hashes are not equal.  Similarly, once one string (say $x$) ends, the hashes are unequal unless $y$ ends at the same time.
%
%A key observation to the following lemmas is that we can look at $T$ not just as a series of transformations, but also as a path through the edit distance dynamic programming table for $x$ and $y$.  In particular, an insert corresponds to taking a ``down'' step in the path, a delete to a ``right'' step, and a ``replace'' to a diagonal step.  If the path reaches a node $(i,j)$ with $x_i = y_j$, the corresponding diagonal is taken automatically---$T$ only denotes choices when $x_i \neq y_j$.  Thus, if $T$ contains $k$ operations, we can view it as a sequence of grid coordinates $(0,0), (i_1,j_1),\ldots,(i_k,j_k)$.

Using the above definition, any transformation induced by $x$, $y$, and $\rho$ corresponds to a sequence of edits that transform $x$ into $y$.
\begin{lemma}
  \lemlabel{transformationcorrect}
  A transformation $T$ induced by any $x$, $y$, and $\rho$ satisfies $T(x,y) = y$.
\end{lemma}
\begin{proof}
  %We begin by proving that any alignment $T$ induced by $x$, $y$, and $\rho$ satisfies $T(x,y) = y$.  
  As above, let $i(x,k,\rho)$ and $i(y,k,\rho)$ be the index of $x$ and $y$ respectively when the $k$th hash character is written.
  We prove the lemma by induction on $k$ in the following claim: the alignment $T_k$ produced by the first $k$ hash characters satisfies $T_k(x[i(x,k,\rho)],y[i(x,k,\rho)]) = y[i(x,k,\rho)]$.   This is trivially satisfied for $k = 0$.  

  Assume that $T_{k-1}(x[i(x,k-1,\rho)],y[i(x,k-1,\rho)]) = y[i(x,k-1,\rho)]$.  We split into three cases based on the operation appended to $T_{k-1}$ to obtain $T_k$.  
  \begin{itemize}
    \item[Case 1:] If a ``replace'' is appended, both $x_i$ and $y_j$ have a hash-replace.  Thus, $i(x,k,\rho) = i(x,k-1,\rho) + 1$, and $i(y,k,\rho) = i(y,k-1,\rho) + 1$.  When the transformation is applied, $x_{i(x,k,\rho)}$ will be replaced with $y_{i(y,k,\rho)}$; thus the final character of $T_{k}(x[i(x,k,\rho)],y[i(y,k,\rho)]) = y[i(y,k,\rho)]$.  We have assumed that the remaining characters are the same by induction.
    \item[Case 2:] If a ``delete'' is appended, $x_i$ has a hash-replace and $y_j$ has a hash-insert.  This means that $i(x,k,\rho) = i(x,k-1,\rho) + 1$, and $i(y,k,\rho) = i(y,k-1,\rho)$.  Applying $T_k$ to $x[i(x,k,\rho)]$ deletes the last character and obtains $T_{k-1}(x[i(x,k-1,\rho],y[i(y,k-1,\rho)])$.  By induction, $T_k(x[i,k,\rho],y[i,k,\rho]) = y[i,k-1,\rho] = y[i,k,\rho]$.
    \item[Case 3:] If an ``insert'' is appended, $x_i$ has a hash-insert and $y_j$ has a hash-replace.  This means that $i(x,k,\rho) = i(x,k-1,\rho)$, and $i(y,k,\rho) = i(y,k-1,\rho)+1$.  Applying $T_k$ to $x[i(x,k,\rho)]$ appends $y_{i(y,k,\rho)}$ and obtains $T_{k-1}(x[i(x,k-1,\rho],y[i(x,k-1,\rho)])\circ y_{i(y,k,\rho)}$.  By induction, $T_k(x[i,k,\rho],y[i,k,\rho]) = y[i,k-1,\rho]\circ y_{i(y,k,\rho)} = y[i,k,\rho]$.\qedhere
  \end{itemize}
\end{proof}

%The correspondence between induced transformations and matching hash strings is formalized in the following lemma. 
Furthermore, the following lemma shows that there is an induced transformation exactly when $x$ and $y$ have the same hash value.  

\begin{lemma}
  \lemlabel{inducesmeanshashes}
  %For any $x$, $y$, and $\rho$, $h_{\rho}(x) = h_{\rho}(y)$ if and only if the alignment $T$ induced by $x$, $y$, and $\rho$ satisfies $T(x,y) = y$.
  %Let $T$ be the alignment induced by some $x$, $y$, and $\rho$.  Then 
  Consider any $x$, $y$, and $\rho$.  
  There exists a transformation $T$ induced by $x$, $y$, and $\rho$  if and only if $h_{\rho}(x) = h_{\rho}(y)$.   
  %Any transformation $T$ induced by $x$, $y$, and $\rho$ satisfies $T(x,y) = y$. 
  %if $h_{\rho}(x) = h_{\rho}(y)$ and $T$ is induced by $x$, $y$, and $\rho$, then $T(x,y) = x$.  
\end{lemma}
\begin{proof}
  Again let $i(x,k,\rho)$ be the index of $x$ when the $k$th character of $h_\rho(x)$ is written.  

  \textbf{If direction}: 
  Assume that $h_{\rho}(x) = h_{\rho}(y)$; we show that there is a transformation $T$ induced by $x$, $y$, and $\rho$.  Assume the contrary: that there is no transformation $T$.  This must be because either $|h_{\rho}(x)| \neq |h_{\rho}(y)|$ (which we can rule out immediately), or there is a $k^*$ (setting $i^* := i(x,k^*,\rho)$ and $j^* := i(y,k^*,\rho)$ for simplicity) with $x_{i^*} \neq y_{j^*}$, but $x_{i^*}$ or $y_{j^*}$ have a hash-match.  Assume that $x_{i^*}$ has a hash-match; the case with $y_{j^*}$ is analogous.  Since $x_{i^*}$ has a hash-match, $x_{i^*}$ is appended onto the output string of $x$.  The next character appended to the output string of $y$ must be either $\bot$ or $y_{j^*} \neq x_{i^*}$; thus the $k^*$th character of the hash of $x$ differs from the $k^*$th character of the hash of $y$, a contradiction.  


\textbf{Only if direction}: 
Assume that there exists a $T$ induced by $x$, $y$, and $\rho$.  We show that each time we add a character to $h_\rho(x)$ and $h_{\rho}(y)$, we add the same character to each.

  First, consider an operation in which we add the $k$th character to $h_\rho(x)$ and $h_\rho(y)$, but we do not add a character to $T$.  Let $x_{i^*}$ be the current character of $x$ and $y_{j^*}$ be the current character of $y$; thus $i^* = i(x,k,\rho)$ and $j^* = i(y,k,\rho)$.  Since we do not add any operation to $T$, either $x_{i^*}$ and $y_{j^*}$ have a hash-insert, or $x_{i^*} = y_{j^*}$.  If $x_{i^*}$ and $y_{j^*}$ have a hash-insert, then $\bot$ is appended to both output strings.  If $x_{i^*} = y_{j^*}$, then $\rho(x_{i^*},k) = \rho(y_{j^*},k)$.  Thus, either $x_{i^*} = y_{j^*}$ is added to both strings, or $\bot$ is added to both strings.  

  Now, consider an operation in which we do add a character to $T$.    
  By \defref{inducedtransformations}, both strings have either a hash-insert or hash-replace; in either case $\bot$ is added to both output strings. 
\end{proof}

\paragraph{Random Walk in the Dynamic Programming Table}
We briefly describe how the above process can be equivalently viewed as a random walk in the edit distance dynamic programming table.  We do not use this view in our analysis; it is presented as an alternative way to understand how the hash function works.

Fix two strings $x$ and $y$.  Consider a directed graph with $(|x|+1)(|y|+1)$ nodes. We label each node using two-dimensional coordinates $(i,j)$ with $0\leq i\leq |x|$, and $0\leq j\leq |y|$.

We now list all arcs between nodes.  
Consider an $(i,j)$ with $0\leq i\leq |x|-1$ and $0\leq j\leq |y|-1$.  For any $(i,j)$ with $x_i = y_j$, we place an arc from $(i,j)$ to $(i+1,j+1)$ of weight 1.  For any $(i,j)$ with $x_i\neq y_j$, we place three arcs of weight $p$: from $(i,j)$ to $(i+1,j)$, from $(i,j)$ to $(i+1,j+1)$, and from $(i,j)$ to $(i,j+1)$.  
There is also an arc from $(|x|,j)$ to $(|x|,j+1)$ for $0\leq j\leq |y|-1$, and from $(i,|y|)$ to $(i,|y|+1)$ for $0\leq i\leq |x|-1$.

We give an example of this graph in TODO.

In a weighted random walk on the graph, the walk traverses an outgoing edge of weight $w$ with probability $w$.  In particular, let $w_1,\ldots w_o$ be the probabilities of all $o$ outgoing arcs for a node $(i,j)$.  The path traverses arc $\ell$ with probability $w_\ell$.  With probability $1 - \sum w_\ell$, the path \defn{dies} and does not traverse any further nodes.  Note that this definition only makes sense if $\sum w_\ell \leq 1$ for all nodes; this is satisfied by the above graph because $p\leq 1/3$ and all nodes have outdegree at most $3$.

\begin{lemma}
  Let $G(x,y)$ be the graph defined above for strings $x$,$y$. Let $p_G(x,y)$ be the probability that a random walk on $G$ dies at node $(|x|+1,|y|+1)$.
  Then $\Pr(h_{\rho}(x) = h_{\rho}(y)) = p_G(x,y)$. 
\end{lemma}
\begin{proof}
  TODO
\end{proof}

The concept of a path ``dying'' in the above definition is unusual for random walks in graphs.  We can reduce this to the standard random walk definition by adding a special sink node representing the \die{} state.  Each other node in the graph with outgoing arc weights $w_1,\ldots, w_o$ is augmented with an additional outgoing arc to the sink node with weight $1 - \sum w_i$.   Using this reduction, random walks do not die; instead, every random walk in the graph ends in the death state, or at node $(|x|+1,|y|+1)$. 


%this is from another part of the paper: 


\begin{lemma}
  \lemlabel{probinducesupper}
  %For any transformation $T$ of length $t$, and for all strings $x$ and $y$,  the probability (over $\rho$) that $\rho$, $x$, and $y$ induce $T$ is at most $p^t$. 
  % $h_{\rho}$ induces $T$ on $x$ and $y$ with probability $p^t$.  
  Let $T$ be a transformation of length $t$ such that $T(x,y) = y$.  Then
  \[
    \Pr_\rho[T = \calT(x,y,\rho)] \leq p^t.
  \]
\end{lemma}
\begin{proof} 
  For any $\rho$ such that  $x$ and $y$  have an alive transformation $T = \calT (x,y,\rho)$, they also have an alive $g(x,y,\rho)$.  For any prefix $T[i]$ of length $i$, we show by induction on $i$ that the probability that $T[i]$ is a prefix of $\calT (x,y,\rho)$ is at most $p^i$. The base case $i=0$ is immediate since $p^0 = 1$.

  Assume that, for all $x'$ and $y'$, the probability that $T[i-1]$ is a prefix of $\calT (x',y',\rho)$ is $p^{i-1}$.  Let $\sigma = T_i$, and  (since $\calT (x,y,\rho)$ is a subsequence of $g(x,y,\rho)$) let $i^*$ be the position in $g(x,y,\rho)$ corresponding to $T_{i-1}$.  
  Then $\sigma$ is the $i$th character in $\calT (x,y,\rho)$ if and only if there exists a $j > i^*$ such that $g_j(x,y,\rho) = \sigma$, and for all $i^* < j' < j$, $g_{j'}(x,y,\rho) = \loo{}$ or $g_{j'}(x,y,\rho) = \match{}$.

  We begin by bounding the probability that $g_{j'}(x,y,\rho)$ is \match{} or \loo{} for all $i^* < j' < j$.  
  %Note that this probability is $1$ for $j'$ satisfying $x_{i(x,j',\rho)} = y_{i(y,j',\rho)}$. 
  Let $J' = \{j' > i^*| x_{i(x,j',\rho)} \neq y_{i(y,j',\rho)}\}$.  Note that $g_{j'}(x,y,\rho)$ is \match{} or \loo{} with probability 1 for $j'\notin J$ if $i^* < j' < j$.  

By \tabref{gridwalk}, for $j'\in J'$, $g_{j'}(x,y,\rho) = \loo{}$ if and only if $\tau_{j'}(x,\rho) = \text{hash-insert}$, and $\tau_{j'}(y,\rho) = \text{hash-insert}$.  These each occur independently with probability $p_a$.
%  We prove this lemma by induction on $t$.  The base case $t=0$ is trivially satisfied.
%
%  Let $T$ be a transformation of length $t+1$, and let $x$ and $y$ satisfy $T(x,y) = y$ (otherwise $x$ and $y$ cannot induce $T$ for any $\rho$, by \lemref{transformationcorrect}).  We split into three cases based on the last operation in $T$. Let $T' = T[t]$, $x' = x[|x|-1]$, and $y' = y[|y|-1]$.  
%  %If strings $x$ and $y$ and underlying function $\rho$ induce $T$, then there exist strings $x'$ and $y'$ such that $x'$, $y'$, and $\rho$ induce the prefix $T[t]$.  In particular, by \defref{inducedtransformations}, $T$ is induced if and only if $x'$ and $y'$ 
%%Assume that all transformations with length $t-1$ are induced for $x$ and $y$ with probability at most $p^{t-1}$.  Consider a transformation $T$ of length $t-1$ for strings $x[i]$ and $y[j]$, and let $T_i$, $T_d$, and $T_r$ be the result of adding an insert, a delete, and a replace to $T$ respectively.  We will show that the probability of each of $T_i$, $T_d$, and $T_r$ 
%  %and let $T'$ be the prefix of $T$ of length $t-1$.  We split into three cases based on the last operation in $T$.
%\begin{itemize}
%  \item[Insert:] By TODO, we must have $T'(x,y') = y'$.  
%    By \defref{inducedtransformations}, $T$ can only be induced on $x$ and $y$ under $\rho$ if $T'$ is induced on $x$ and $y'$ under $\rho$, $x_i$ has a hash-insert, and $y_j$ has a hash-replace.
%    By the inductive hypothesis, $T'$ is induced on $x$ and $y'$ under $\rho$ with probability $p^t$.
%  \item[Delete:] By TODO, we must have $T'(x',y) = y$. 
%  \item[Replace:] By TODO, we must have $T'(x',y')=y'$.  
%\end{itemize}
%  %This means that in \defref{inducedtransformations}, for all $i$ and $j$ we must either have $x_i = y_j$, or both $x_i$ and $y_j$ have a hash-replace.  However, if $x_i$ and $y_j$ have a hash-replace, then $i$ and $j$ do not increment.  
\end{proof}


==> oldtightupper.tex <==

\subsection{Bounds on Collision Probabilities}

\begin{lemma}
  \lemlabel{closepoints}
  If $x$ and $y$ satisfy $\ED(x,y) \leq r$, then 
  \[
    \Pr_{h\in \calH} (h(x) = h(y)) \geq p^r
  \]
\end{lemma}

\begin{proof}
  Because $\ED(x,y)\leq r$, there exists a transformation $T$ of length $r$ such that $T(x) = y$.  By \lemref{probinduces}, $h$ induces $T$ on $x$ and $y$ (which is sufficient for $h(x) = h(y)$ by \lemref{inducesmeanshashes}) with probability $p^r$.  
\end{proof}

%We show the following upper bound on collision probabilities.  

TODO: fix this to work with all paths of length $> x$ for any $x$.

\begin{lemma}
  \lemlabel{looseupper}
  If $x$ and $y$ satisfy $\ED(x,y) \geq cr$, then 
  \[
    \Pr_{h\in \calH} (h(x) = h(y)) \leq (3p)^{cr}
  \]
\end{lemma}

\begin{proof}
  Let $\calT$ be the set of all transformations that align $x$ and $y$; i.e. $\calT = \{T | T(x) = y\}$.  By 
  \lemref{inducesmeanshashes} and 
  \lemref{probinduces}, 
  \[
    \Pr_{h\in \calH} (h(x) = h(y)) = \sum_{T\in \calT} p^{|T|}.
  \]
Thus, we want to find the $\calT$ (for the given $x$ and $y$) that maximizes this probability.
  
  By \lemref{prefixfree}, there is no pair $T_1, T_2\in \calT$ such that $T_1$ is a prefix of $T_2$.  Thus, $\calT$ can be viewed as the leaves of a trie of branching factor at most $3$, where each leaf has depth at least $cr$.  
  
  %TODO: each non-costly edge in the trie has branching factor at most 1, so they can be collapsed; this means the cost of a leaf is exactly its depth.  
  
  %Consider a nodes of the trie at depth $cr$ (if any does not exist, we can increase the collision probability of $S$ by adding paths to these nodes in the trie).  Consider
  We show that without loss of generality all leaves are at depth $cr$.  Consider a leaf $T_1$ at the maximum depth of the trie $i > cr$, and its siblings $T_2$ and $T_3$ if they exist.  Collapse this leaf and its siblings, replacing them instead with a leaf $T_p$ corresponding to their parent in the trie; call the resulting set $\calT'$.  Since we have added a transformation of length $i-1$ and removed at most three of length $i$, this  changes the total cost of $\calT$ by at least $p^{i-1} - 3p^{i}$; this is positive since $p \leq 1/3$.
  %\begin{align*}
  %  \sum_{s\in S'} p^{\text{cost}(s)} &= \left(\sum_{s\in S} p^{\text{cost}(s)}\right) - p^{\text{cost}(s_1)} - p^{\text{cost}(s_2)} - p^{\text{cost}(s_3)} + p^{\text{cost}(s_p)}\\
  %  &\geq \sum_{s\in S} p^{\text{cost}(s)}
  %\end{align*}
Repeating this process results in a set $\calT_M$ with all nodes at depth $cr$, where $\calT_M$ gives larger collision probability than the original set $\calT$.  

  There are at most $3^{cr}$ transformations in $\calT_M$, each of length $cr$.  Thus
  \[
    \Pr_{h\in \calH} (h(x) = h(y)) \leq 3^{cr} p^{cr}.\qedhere
  \]
\end{proof}

With the above, we can give a tight upper bound on the probability that two far elements collide.

\begin{lemma}
  \lemlabel{tightupper}
  If $x$ and $y$ satisfy $\ED(x,y) \geq cr$, then 
  \[
    \Pr_{h\in \calH} (h(x) = h(y)) \leq (cr)^2\left(\frac{2p}{1-p}\right)^{cr}.
  \]
\end{lemma}

\begin{proof}
  We say that a match is \defn{significant} (for a cost $cr$) if 
  item either its left neighbor or upper neighbor 
      a) is not a match, and 
      b) has cost at most $2cr$.  

  Let $T_{2cr}(\ell,k,m,m_s)$ be the total weight of all transformations from the first $\ell$ letters of $x$ to the first $k$ letters of $y$ (in other words, $\ell$ total steps down and $k$ total steps right in the dynamic programming table) which traverse $m$ total matches, $m_s$ significant matches, and have length at most $2cr$.\footnote{This proof can be completed using $m$ as the total number of match steps overall, skipping the concept of ``significant'' and not requiring \lemref{TODO}.  However, this would lead to a leading $d$ term in the final bound.}

  By \lemref{TODO}, all paths of length at least $2cr$ have cost
  \[
    (3p)^{2cr} \leq \left(\frac{2p}{1-p}\right)^{cr}
  \]

  TODO: figure showing what this means.

  Summing the weight of transformations of length at least $cr$, and transformations of length at most $cr$, and letting $d_{\max} = \max\{|x|,|y|\}$, we have 
  \[
    \Pr_{h\in\calH} (h(x)=h(y)) \leq \left(\frac{2p}{1-p}\right)^{cr} +  \sum_{m = d_{\max} - 2cr}^{d_{\max} -cr} \sum_{m_s = 0}^{m} T(|x|,|y|,m,m_s).
  \]

  We bound $T(\ell,k,m,m_s)$ recursively.  First, assume that $(\ell,k)$ is not a match.  Then 
  \[
    \text{\textbf{(Case 1):}} \qquad T(\ell,k,m,m_s) \leq pT(\ell - 1,k,m,m_s) + pT(\ell,k-1,m) + pT(\ell-1,k-1,m,m_s). 
  \] 
  Next, if $(\ell,k)$ is a significant match, then 
  \[
    \text{\textbf{(Case 2):}} \qquad T(\ell,k,m,m_s) \leq pT(\ell - 1,k,m,m_s) + pT(\ell,k-1,m,m_s) + T(\ell-1,k-1,m-1,m_s - 1). 
  \] 
  Finally, if $(\ell,k)$ is a match but it is not significant, then its upper and left neighbor are either a match, or have cost at least $2cr$.  If they are a match, then they do not contribute to $T(\ell,f,m,m_s)$ by TODO.  If they have cost at least $2cr$, then they do not contribute to $T(\ell,f,m,m_s)$ because all paths through that node have cost at least $2cr$.  Therefore, in this case, 
  \[
    \text{\textbf{(Case 3):}} \qquad T(\ell,k,m,m_s) = T(\ell-1,k-1,m-1,m_s). 
  \] 

  We bound this recurrence using an induction on the grid. 
  The desired bound is
  \[
    T(\ell,k,m,m_s) \leq \left\{ \begin{array}{lr} m_s(2p/(1-p)))^{\ell - m} & \text{if $\ell \geq k$}  \\ m_s(2p/(1-p))^{k-m} & \text{ otherwise.} \end{array}\right.
  \]
  The base case with $k = 0$ or $\ell = 0$ (implying $m = 0$) is obvious from TODO, as there is only one transformation. 


  Assume that $\ell \geq k$ (the proof for $\ell < k$ is identical with $\ell$ and $k$ switched). 

  \textbf{Case 1:} Substituting our upper bound in the recursive terms, we obtain one of two bounds.  If $\ell > k$, 
  \begin{align*}
    T(\ell,k,m,m_s) &\leq p m_s(2p/(1-p))^{\ell-m-1} + 2p m_s(2p/(1-p))^{\ell-m} \\
                    &\leq  ((1-p)/2 + 2p) m_s(2p/(1-p))^{\ell - m} \\
                    &\leq  m_s(2p/(1-p))^{\ell-m},
  \end{align*}
  where the last step is from $p < 1/3$. The case where $\ell = k$ is essentially the same: 
  \begin{align*}
    T(\ell,k,m,m_s) &\leq p m_s(2p/(1-p))^{\ell-m-1} + p m_s(2p/(1-p))^{k-m-1} + p m_s(2p/(1-p))^{\ell-m} \\
                    &\leq  ((1-p)+ p) m_s(2p/(1-p))^{\ell - m} \\
                    &\leq  m_s(2p/(1-p))^{\ell-m}. 
  \end{align*}
  In both cases, our inductive assumption holds.  

  \textbf{Case 2:} Again substituting, if $\ell \neq k$,  
  \begin{align*}
    T(\ell,k,m,m_s) &\leq p m_s(2p/(1-p))^{\ell-m-1} + p m_s(2p/(1-p))^{\ell-m} + (m_s - 1) (2p/(1-p))^{\ell - m}\\
                    &\leq  ((1-p)/2 + p - 1) m_s(2p/(1-p))^{\ell - m} + m_s(2p/(1-p))^{\ell - m} \\
                    &\leq  m_s(2p/(1-p))^{\ell-m}.
  \end{align*}
  The $-1$ in the first term in step 2 comes from the $(m_s - 1)$ term in step 1.
\end{proof}



%OLDER


\subsection{A Tight Upper Bound}

In this section, we show a tight bound on the worst-case collision probability between two elements at distance $cr$.  

\begin{lemma}
  \lemlabel{tightupper}
  If $x$ and $y$ satisfy $\ED(x,y) \geq cr$, then 
  \[
    \Pr_{h\in \calH} (h(x) = h(y)) \leq O\left(\left(\frac{2p}{1-p}\right)^{cr}\right).
  \]
\end{lemma}



The following lemma shows that this bound is tight up to lower-order terms.

\begin{lemma}
  \lemlabel{uppertight}
  Assume $cr$ is even.  
  Let 
  $\hat{x} = 0^{cr/2} 1^{cr/2}$ and  $\hat{y} = 1^{cr/2} 0^{cr/2}$. 
  Then $\ED(\hat{x},\hat{y}) = cr$, and
  \[
    \Pr_{h\in \calH} (h(\hat{x}) = h(\hat{y})) \geq \frac{4}{9(cr)^2} \left(\frac{2}{1-p}\right)^{cr}
  \]
\end{lemma}

\begin{proof}
  Consider the total cost of all nodes $i,j$ with distance $k$; call this $C(k)$.  By TODO, this can be written as the sum of the cost of all transformations ending at each $i,j$:
  \[
    C(k) = \sum_{i,j \text{ distance } k} \sum_{T \text{ ends at } i,j; \text{length } \ell} p^{\ell}.
  \]

  Consider a transformation $T$ ending at a given node $(i,j)$ at distance $j$, with $i < j < cr/2$.  Then there exists two transformations $T_1$ and $T_2$ ending at a node with distance $j+1$, and a transformation $T_3$ ending at a node with distance $j$, where $T_1$, $T_2$, and $T_3$ consist of $T$ with one operation appended.  A similar argument applies to nodes $(j,i)$ at distance $j$, with $i < j < cr$.  
  
  Finally, consider a transformation $T$ ending at $(j,j)$.   Then there are three transformations $T_1, T_2, and T_3$ ending at a node with distance $j+1$. Again, each consists of $T$ with one operation appended.

  Putting the above together, $ C(k) \geq 2pC(k-1) + pC(k)$ for $k < cr/2$, and $C(k) \geq 2pC(k-1)$ for $k = cr/2$.  Since $C(1) = 1$, we obtain that 
  \[
    C(cr/2) \geq (1-p)\left(\frac{2p}{1-p}\right)^{cr/2}
  \]
  There are at most $cr$ nodes at distance $cr/2$.   
  Thus, there exists a node $(i^*,cr/2)$ with cost at least 
  \[
    \frac{1-p}{cr}\left(\frac{2p}{1-p}\right)^{cr/2}
  \]

  Now, we consider the cost of all transformations $T$ TODO: matching the hash AND going through $(i^*,cr/2)$.  By examination, we can see that this is exactly the cost of node $(cr/2,i^*)$; by symmetry, this is equal to the cost of $(i^*,cr/2)$.  Thus the total costs of all transformations passing through $(i^*,cr/2)$ is at least 
  \[
    \left(\frac{1-p}{cr}\right)^2 \left(\frac{2p}{1-p}\right)^{cr}.
  \]
  Substituting $p \leq 1/3$ we obtain the lemma.
\end{proof}

The \defn{Ulam} metric is the edit distance on permutations---in other words, the Ulam metric is the same as edit distance but restricted to strings with alphabet $|\Sigma| = d$ and no repeated characters.  Previous work has shown stronger bounds under the Ulam metric than for edit distance: in particular for embeddings~\cite{CharikarKrauthgamer06}, but also for approximation algorithms~\cite{AndoniNguyen10,NaumovitzSaSe17}.  Unfortunately, for our LSH the above analysis is tight for the Ulam metric as well as edit distance.

\begin{corollary}
  \corlabel{uppertightulam}
  There exist two strings $\hat{x}$ and $\hat{y}$ at distance $cr$ under the Ulam metric that have collision probability 
  \[
    \Pr_{h\in \calH} (h(\hat{x}) = h(\hat{y})) \geq \frac{4}{9(cr)^2} \left(\frac{2}{1-p}\right)^{cr}
  \]
\end{corollary}
\begin{proof}
  The high-level goal of this proof is to create two strings under the Ulam metric such that the cost of all paths passing through $(i^*,cr/2)$ remains unchanged---thus, the analysis of \lemref{uppertight} still holds.  We assume that $\Sigma = \{1,\ldots,d\}$. 

  Assume without loss of generality that $\hat{x} = 123\ldots d$. We concatenate three strings to obtain $\hat{y}$.  We momentarily abuse notation by using a comma to denote concatenation of characters. The first $cr/2$ characters of $\hat{y}$ are $cr/2+1, cr/2+2,\ldots, cr$. The following $i^*$ characters are $i^*, i^* + 1,\ldots, 2i^*$.  The remaining $cr - i^*$ characters are $1,2,\ldots, cr-i^*$.  

  As shown in Figure TODO, these strings retain all paths through $(i^*,cr/2)$, and edit distance $cr$. 
\end{proof}
\fi


==> omittedproofs.tex <==
\section{Omitted Proofs}
\seclabel{omittedproofs}

\begin{proofof}{\lemref{shorthash}}
  If $\tau(x,\rho)$ has $\ell$ hash-insert operations, then $|\tau(x,\rho)| \leq d + \ell$.  We bound the probability that $\ell > 7d/(1 - p_a) + 6\log n$.

  For each character in $x$, we can model the building of $\tau(x,\rho)$ as a series of independent coin flips. On heads (with probability $p_a$), $\ell$ increases; on tails the process stops.  Thus we expect $1/(1-p_a)$ hash-insert operations for each character of $x$, and at most $d/(1 - p_a)$ hash-insert operations overall.

  Using standard Chernoff bounds (i.e.~\cite[Exercise 4.7]{MitzenmacherUpfal17}), the probability that $\ell > 7d/(1 - p_a) + 6\log n$ is at most $\exp((6d(1-p_a) + 6\log n)/3) < 1/n^2$.
  %For each $k$, $\Pr[\tau_k(x,\rho) = \text{ hash-insert}] = p_a$; these probabilities are independent.  Therefore, the expected number of hash-insert operations is $d/(1-p_a)$.
\end{proofof} 

\bigskip

\begin{proofof}{\lemref{walkcorrectness}}
Our proof is by induction on $k$.  We prove both that the walk arrives at node $(i(x,k,\rho),i(y,k,\rho))$, and that the walk is well-defined: the next character in $g(x,y,\rho)$ always corresponds to an outgoing edge of the current node.   

    For the base case $k = 0$ the proof is immediate, since $(i(x,0,\rho),i(y,0,\rho)) = (0,0)$.  Furthermore, node $(0,0)$ has an outgoing \match{} edge if and only if $x_0 = y_0$ (otherwise it has an outgoing \ins{}, \del{}, and \rep{} edge); similarity, $g_0(x,y,\rho) = \match{}$ only if $x_0 = y_0$ (the rest of the cases follow likewise). 

    Assume that after $k-1$ steps, the walk using $g(x,y,\rho)[k-1]$ arrives at node $(i(x,k-1,\rho),i(y,k-1,\rho))$.  We begin by proving that the walk remains well-defined.  We have $g_{k-1}(x,y,\rho) = \match{}$ only if $x_{i(x,k-1,\rho)} = y_{i(y,k-1,\rho)}$; in this case $(i(x,k-1,\rho),i(y,k-1,\rho))$ has an outgoing \match{} edge.  We have $g_{k-1}(x,y,\rho) = \ins{}$ (or \del{} or \rep{}) only if $x_{i(x,k-1,\rho)} \neq y_{i(y,k-1,\rho)}$; again, node $(i(x,k-1,\rho),i(y,k-1,\rho))$ has the corresponding outgoing edge.  All nodes have outgoing \loo{} and \die{} edges.

    Now we show that after $k$ steps, the walk using $g(x,y,\rho)[k]$ arrives at node $(i(x,k,\rho),i(y,k,\rho))$.  We split into five cases based on $g_{k-1}(x,y,\rho)$ (if $g_{k-1}(x,y,\rho) = \die{}$ the lemma no longer holds).
    \begin{itemize}
      \item[\rep{}] We have $\tau_k(x,\rho) = $ hash-replace, and $\tau_k(y,\rho) = $ hash-replace.  Thus, $i(x,k,\rho) = i(x,k-1,\rho) + 1$ and $i(y,k,\rho) = i(y,k-1,\rho) + 1$.  In $G(x,y)$, the edge labelled \rep{} leads to node $(i(x,k-1,\rho)+1,i(y,k-1,\rho) + 1)$.
      \item[\match{}] We have $\tau_k(x,\rho) = $ hash-replace, and $\tau_k(y,\rho) = $ hash-replace.  Thus, $i(x,k,\rho) = i(x,k-1,\rho) + 1$ and $i(y,k,\rho) = i(y,k-1,\rho) + 1$.  In $G(x,y)$, the edge labelled \match{} leads to node $(i(x,k-1,\rho)+1,i(y,k-1,\rho) + 1)$.
      \item[\del{}] We have $\tau_k(x,\rho) = $ hash-replace, and $\tau_k(y,\rho) = $ hash-insert.  Thus, $i(x,k,\rho) = i(x,k-1,\rho) + 1$ and $i(y,k,\rho) = i(y,k-1,\rho)$.  In $G(x,y)$, the edge labelled \ins{} leads to node $(i(x,k-1,\rho)+1,i(y,k-1,\rho))$.
      \item[\ins{}] We have $\tau_k(x,\rho) = $ hash-insert, and $\tau_k(y,\rho) = $ hash-replace.  Thus, $i(x,k,\rho) = i(x,k-1,\rho)$ and $i(y,k,\rho) = i(y,k-1,\rho)+1$.  In $G(x,y)$, the edge labelled \ins{} leads to node $(i(x,k-1,\rho),i(y,k-1,\rho)+1)$.
      \item[\loo{}] We have $\tau_k(x,\rho) = $ hash-insert, and $\tau_k(y,\rho) = $ hash-insert.  Thus, $i(x,k,\rho) = i(x,k-1,\rho)$ and $i(y,k,\rho) = i(y,k-1,\rho)$.  In $G(x,y)$, the edge labelled \loo{} leads to node $(i(x,k-1,\rho),i(y,k-1,\rho))$.\qedhere
    \end{itemize}
\end{proofof}

\bigskip

  \begin{proofof}{\lemref{walkcollision}}
    \ifdirection Assume that $h_{\rho}(x) = h_{\rho}(y)$; we show that the path defined by $g(x,y,\rho)$ is alive and reaches $(|x|,|y|)$. 
    
    First, $g(x,y,\rho)$ must be alive: $g_k(x,y,\rho) = \die{}$ only when $x_{i(x,k,\rho)} \neq y_{i(y,k,\rho)}$ and either $\tau_k(x,\rho) = $ hash-match or $\tau_k(y,\rho) = $ hash-match, or when $k > \min\{|\tau(x,\rho)|,|\tau(y,\rho)|\}$. Since $x_{i(x,k,\rho)}$ (resp. $y_{i(y,k,\rho)}$) is appended to the hash on a hash-match, this contradicts $h_{\rho}(x) = h_{\rho}(y)$.  Furthermore, we must have $|\tau(x,\rho)| = |\tau(y,\rho)|$ because 
    %by \obsref{transcripthashlength},
    $|\tau(x,\rho)| = |h_{\rho}(x)| = |h_{\rho}(y)| = |\tau(y,\rho)|$.  

    Since $\tau(x,\rho)$ and $\tau(y,\rho)$ are complete, 
    %By \obsref{completeindex}, 
    $i(x,|\tau(x,\rho)|-1,\rho) = |x|$ and $i(y,\tau(y,\rho)-1,\rho) = |y|$.  Thus, by \lemref{walkcorrectness}, the walk reaches $(|x|,|y|)$.  

    \onlyifdirection We show that if $h_{\rho}(x) \neq h_{\rho}(y)$ then $g(x,y,\rho)$ is not alive.  Let $k$ be the smallest index such that the $k$th character of $h_{\rho}(x)$ is not equal to the $k$th character of $h_{\rho}(y)$.  At least one of these characters cannot be $\bot$; thus either $\tau_k(x,\rho) = $ hash-match, or $\tau_k(y,\rho) = $ hash-match.  If $x_{i(x,k,\rho)} \neq y_{i(x,k,\rho)}$, then $g_k(x,y,\rho) = \die{}$ and we are done.  Otherwise, $x_{i(x,k,\rho)} = y_{i(y,k,\rho)}$; thus $\tau_k(x,\rho) = \tau_k(y,\rho)$, and the $k$th character of both $h_{\rho}(x)$ and $h_{\rho}(y)$ is $x_{i(x,k,\rho)} = y_{i(y,k,\rho)}$.  But this contradicts the definition of $k$. 
  \end{proofof}

  \bigskip

  \begin{proofof}{\lemref{gridwalkprobs}}
  We have $|\tau(x,\rho)| > k$ and $|\tau(y,\rho)| > k$ from $E_k$.  
  Thus: 
  \begin{itemize}[topsep=0pt,noitemsep]
    \item $\Pr_\rho(\tau_k(x,\rho) = \text{hash-insert} ~|~ E_k) = p_a$
    \item $\Pr_\rho(\tau_k(x,\rho) = \text{hash-replace} ~|~ E_k) = (1-p_a)p_r$
    \item $\Pr_\rho(\tau_k(x,\rho) = \text{hash-match} ~|~ E_k) = (1-p_a)(1-p_r)$.
  \end{itemize}
  The respective probabilities for $\tau_k(y,\rho)$ hold as well.
  Combining these probabilities with \tabref{gridwalk} gives the lemma.  
  \end{proofof}

  \bigskip

 \begin{proofof}{\lemref{transformationfromED}}
   We prove a single statement implying the lemma: if $\hat{T}$ is the shortest transformation that solves $x\concat\$ $ and $y\concat\$ $, then $|\hat{T}| = \ED(x,y)$.

   %Assume the contrary; let $T'$ be the shortest transformation that satisfies $T'(x\concat\$,y\concat\$)$, and let $|T'| < r$. 
   Let $\sigma_1,\ldots \sigma_r$ be the sequence of edits applied to $x\concat\$ $ to obtain $\hat{T}(x\concat\$,y\concat\$)$ in \defref{transformation}.  These operations apply to increasing indices $i$ because $\hat{T}$ is the shortest transformation satisfying $\hat{T}(x\concat\$,y\concat\$)$.  Let $\sigma_i$ be the last operation that applies to an index $i < |x|$. Let $\hat{y} = \hat{T}[i+1](x\concat\$,y\concat\$)$ be the string obtained after applying the operations of $\hat{T}$ through $\sigma_i$.  Clearly, $x$ is a prefix of $\hat{y}$.  
   We claim that because $\hat{T}$ is the shortest transformation, the operations in $\hat{T}$ after $\sigma_i$ must be $|\hat{y}| - |x| - 1|$ \ins{} operations.  Clearly there must be at least $|\hat{y} - |x| - 1|$ operations after $\sigma_i$ because $i$ is increasing and only one character in $\hat{y}$ matches the final character $\$$ of $x$.  By the same argument, if $\hat{T}$ has any \ins{} or \rep{} operations it cannot meet this bound.  

   With this we have $\ED(x,y) \leq |\hat{T}|$ because we can apply $\sigma_1,\ldots,\sigma_i$, followed by $|\hat{y} - |x| - 1|$ insert operations to $x$ to obtain $y$.  This totals to $|\hat{T}|$ operations overall.

   We also have $\ED(x,y) \geq |\hat{T}|$ by minimality of $\hat{T}$ because any sequence of edits applied to $x$ that obtains $y$ will obtain $y\concat \$$ when applied to $x\concat\$$.  
\end{proofof}

\bigskip

\begin{proofof} {\lemref{hasheseqtransformation}}
  \ifdirection Assume $T$ solves $x$ and $y$.  Since $x\neq y$, $T$ must be nonempty; thus $g(x,y,\rho)$ is alive.  By \lemref{walkcollision}, $h_\rho(x) = h_\rho(y)$.  

    \onlyifdirection Assume $h_\rho(x) = h_\rho(y)$; by \lemref{walkcollision} $g(x,y,\rho)$ is alive.

    Let $g(x,y,\rho)[k]$ be the prefix of $g(x,y,\rho)$ of length $k$, and let $T^k$ be $g(x,y,\rho)[k]$ with $\loo{}$ and $\match{}$ removed.  We prove by induction that $T^k(x[i(x,k,\rho)],y[i(y,k,\rho)]) = y[i(y,k,\rho)]$.  This is trivially satisfied for $k = 0$.  

    Assume that $T^{k-1}(x[i(x,k-1,\rho)],y[i(y,k-1,\rho)]) = y[i(y,k-1,\rho)]$.  We split into five cases based on the $k$th operation in $g(x,y,\rho)$.
\begin{itemize}
  \item[\match] We must have $x_{i(x,k-1,\rho)} = y_{i(y,k-1,\rho)}$ and $T^k = T^{k-1}$.  Furthermore, $i(x,k,\rho) = i(x,k-1,\rho) + 1$ and $i(y,k,\rho) = i(y,k-1,\rho) + 1$.  Thus $T^{k}(x[i(x,k,\rho)],y[i(y,k,\rho)]) = T^{k-1}(x[i(x,k-1,\rho)],y[i(y,k-1,\rho)])\concat x_{i(x,k-1,\rho)} = y[i(y,k,\rho)]$.  
  \item[\ins] We have $i(x,k,\rho) = i(x,k-1,\rho)$ and $i(y,k,\rho) = i(y,k-1,\rho) + 1$.  Thus, $T^{k-1}(x[i(x,k,\rho)],y[i(y,k,\rho)]) = y[i(y,k-1,\rho)]$ and $y[i(y,k,\rho)]$ differ only in the last character.  Then 
    $T^{k}(x[i(x,k,\rho)],y[i(y,k,\rho)]) = T^{k-1}(x[i(x,k-1,\rho)],y[i(y,k-1,\rho)])\concat y_{i(y,k,\rho)-1} = y[i(y,k,\rho)]$.  

  \item[\rep] We have $i(x,k,\rho) = i(x,k-1,\rho)+1$ and $i(y,k,\rho) = i(y,k-1,\rho) + 1$.  Thus, $T^{k-1}(x[i(x,k,\rho)],y[i(y,k,\rho)]) = y[i(y,k-1,\rho)] \concat x_{i(x,k,\rho)-1}$ and $y[i(y,k,\rho)]$ differ only in the last character.  By definition, the final character of $T^{k-1}(x[i(x,k,\rho)],y[i(y,k,\rho)]$ is replaced with $y_{i(y,k,\rho)-1}$, obtaining $T^k(x[i(x,k,\rho)],y[i(y,k,\rho)]) = y[i(y,k-1,\rho)]\concat y_{i(y,k,\rho)-1} = y[i(y,k,\rho)]$.  
    %Then 

  \item[\del] We have $i(x,k,\rho) = i(x,k-1,\rho)+1$ and $i(y,k,\rho) = i(y,k-1,\rho)$.  Thus, $T^{k-1}(x[i(x,k,\rho)],y[i(y,k,\rho)]) = y[i(y,k-1,\rho)] \concat x_{i(x,k,\rho) - 1}$ and $y[i(y,k,\rho)]$ differ only in the last character (which is deleted). Then 
    $T^{k}(x[i(x,k,\rho)],y[i(y,k,\rho)]) = T^{k-1}(x[i(x,k-1,\rho)],y[i(y,k-1,\rho)]) = y[i(y,k,\rho)]$.  

  \item[\loo] We have $i(x,k,\rho) = i(x,k-1,\rho)$, $i(y,k,\rho) = i(y,k-1,\rho)$, and $T^k = T^{k-1}$.  We immediately obtain $T^k(x[i(x,k,\rho)],y[i(y,k,\rho)]) = y[i(y,k,\rho)]$.  
\end{itemize}
  By \lemref{walkcollision}, $g(x,y,\rho)$ reaches node $(|x|,|y|)$, so the above shows that with $k = |g(x,y,\rho)|$, $T(x,y) = y$.  
    %By \lemref{walkcollision}, the path through $G(x,y)$ defined by $g(x,y,\rho)$ reaches node $(|x|,|y|)$.  
    %In a slight abuse of notation, let $\calT(x,y,\rho)[k]$ be the string obtained by removing $\loo{}$ and $\die{}$ from 
\end{proofof}

\bigskip

\begin{proofof}{\lemref{probinduces}}
%For any transformation $T$, 
  Let $G_T$ be the set of all grid walks $g$ (i.e. the set of all sequences consisting of grid walk operations) such that $g$ does not contain \die{}, and deleting \loo{} and \match{} from $g$ results in $T_g$ such that $T$ is a prefix of $T_g$.  
  Then by definition, if $T$ is a prefix of $\calT(x,y,\rho)$ then $g(x,y,\rho)\in G_T$; furthermore, if $g(x,y,\rho)\in G_T$ and $g(x,y,\rho)$ is complete, then $T$ is a prefix of $\calT(x,y,\rho)$. 
  %Then we can upper bound $\Pr_{\rho}[T = \calT(x,y,\rho)]$ by $\Pr_\rho[g(x,y,\rho) \in G_T]$.  

  %Thus, we aim to prove that 
  We begin by proving that $\Pr_\rho[g(x,y,\rho) \in G_T] = p^t$.  
  We prove this by induction on $t$; $t = 0$ is trivially satisfied.  We assume that $\Pr_\rho[g(x,y,\rho)\in G_{T'}] = p^{t-1}$ for any $G_{T'}$ with $|T'| = t-1$, and prove that it holds for any $T$ with $|T| = t$.

  Let $\sigma$ be the last operation in $T$, and let $T' = T[|T|-1]$ be $T$ with $\sigma$ removed.  
  Thus, $g(x,y,\rho) \in G_T$ only if there exist grid walks $g'$ and $g''$ satisfying %, and $g_2$ with $g(x,y,\rho) = g'\concat \sigma\concat g_1\concat g_2$ satisfying:
  \begin{itemize}[topsep=0pt,noitemsep]
    \item $g' \in G_{T'}$,
    \item $g''$ consists of $\loo{}$ and $\match{}$ operations concatenated onto the end of $g'\concat \sigma$, ending with a $\match{}$ operation, and
    \item $g(x,y,\rho)$ consists of zero or more \loo{} operations concatenated onto $g''$.
  \end{itemize}
%where $g = g'\concat \sigma \concat g_1\concat g_2$. 
  By definition of conditional probability, 
  \[
    %\Pr[g(x,y,\rho) \in G_T] = \Pr[g'\in G_{T'}]\Pr[g'\concat\sigma\in G_T]\Pr[g'\concat\sigma\concat g_1\in G_T]\Pr[g'\concat\sigma\concat
    \Pr[g(x,y,\rho) \in G_T] = \sum_{g'} \Pr[g'\in G_{T'}] \sum_{g''} \Pr[g''\in G_T ~|~ g'\in G_{T'} ]\Pr[g(x,y,\rho)\in G_T ~|~ g''\in G_T].
  \]
  We bound these terms one at a time.

  Clearly there is only one $g'$ satisfying the conditions, which can be obtained by taking the prefix of $g(x,y,\rho)$ before the final $\ins{}$, $\del{}$, or $\rep{}$ operation.  By the inductive hypothesis, $\sum_{g'} \Pr[g'\in G_{T'}] = p^{t-1}$.  

  %such that for some $\ell$ we can append one $\sigma$ operation followed by $\ell$ \loo{} operations (depending on $x$, $y$, and $g$ this may be followed by some \match{} operations interspersed with \loo{} operations; we ignore these operations in our upper bound) to $g'$ to obtain $g$.  
  %Assume that $g'$ reaches $(\hat{i},\hat{j})$ in $G(x,y)$ ($\hat{i}$ and $\hat{j}$ must exist because $g'$ is alive); by \lemref{walkcorrectness}, $\hat{i} = i(x,|g'|,\rho)$ and $\hat{j} = i(y,|g'|,\rho)$.  If $x_{\hat{i}} = y_{\hat{j}}$, then $g\in G_T$ if $g'\in G_T$.  

  %Otherwise, 
  We now bound $\Pr[g''\in G_T ~|~ g'\in G_T]$.  The conditional means that we can invoke \lemref{gridwalkprobs} (as $\Pr[E_k] = p^{t-1} > 0$).  
  
  We have $\Pr[g''\in G_T ~|~ g'\in G_{T'}] = \Pr[g''\in G_T ~|~ g'\concat\sigma\in G_T]\Pr[g'\concat\sigma\in G_T ~|~ g'\in G_{T'}]$.

  We split into two cases depending on $\sigma$.  Recall that $p_r = p_a/(1 - p_a)$.  Since $T$ is valid, if $\sigma = \del{}$ or $\sigma = \rep{}$ we cannot have $i(x,k,\rho) = |x|-1$;  similarly if $\sigma = \ins{}$ or $\sigma = \rep{}$ we cannot have $i(y,k,\rho) = |y| - 1$.  
  Then by \lemref{gridwalkprobs}, if $\sigma = \del{}$ or $\sigma = \ins{}$,
  \[
    \Pr(g'\concat \sigma \in G_T ~|~ g'\in G_{T'}) = p_a(1-p_a)p_r = p_a^2.
  \]
%The last line follows from $p_r = p_a/(1 - p_a)$, and $p_a^2/(1 - p_a^2) = p$.  
Similarly, if $\sigma = \rep{}$, 
  \[
    \Pr(g'\concat \sigma \in G_T ~|~ g'\in G_{T'}) = (1-p_a)^2p_r^2 = p_a^2.
  \]
  For any $k$ such that $i(x,k,\rho) = i(y,k,\rho)$, $g_k(x,y,\rho)\neq \die{}$ by definition; meanwhile, if $i(x,k,\rho) \neq i(y,k,\rho)$ then $g_k(x,y,\rho)\neq \match{}$.  Thus, $\sum_{g''} \Pr(g''\in G_T ~|~ g'\concat\sigma\in G_T) = 1$.
  %\begin{align*}
  %  \Pr(g\in G_T) &\leq \sum_{\ell \geq 0} \Pr(g' \in G_{T'}) p_a^{2\ell} p_a(1-p_a)p_r\\
  %                &\leq p^{t-1} p_a(1-p_a) p_r \sum_{\ell \geq 0} p_a^{2\ell}\\
  %                &\leq p^{t-1}\frac{ p_a(1-p_a) p_r }{1 - p_a^2}\\
  %                &= p^t.
  %\end{align*}
%The last line follows from $p_r = p_a/(1 - p_a)$, and $p_a^2/(1 - p_a^2) = p$.  
%Similarly, if $\sigma = \rep{}$, 
  %\begin{align*}
  %  \Pr(g\in G_T) &\leq \sum_{\ell \geq 0} \Pr(g' \in G_{T'}) p_a^{2\ell} (1-p_a)^2 p_r^2\\
  %                &\leq p^{t-1} (1-p_a)^2 p_r^2 \sum_{\ell \geq 0} p_a^{2\ell}\\
  %                &\leq p^{t-1}\frac{ (1-p_a)^2 p_r^2 }{1 - p_a^2}\\
  %                &= p^t.
  %\end{align*}\qedhere

  Finally we bound $\Pr[g(x,y,\rho)\in G_T ~|~ g''\in G_T]$.  Let $\ell$ be the number of operations concatenated onto $g''$ to obtain $g(x,y,\rho)$.  Then by \lemref{gridwalkprobs}, 
  \[
    \Pr[g(x,y,\rho)\in G_T ~|~ g''\in G_T]  = \sum_{\ell} p_a^{2\ell} = 1/(1 - p_a^2).
  \]

  Multiplying the above bounds, we have $\Pr[g(x,y,\rho) \in G_T] = p^{t-1}p_a^2/(1 - p_a^2)$.  Noting that $p = p_a^2/(1 - p_a^2)$, we obtain $\Pr[g(x,y,\rho)\in G_T] = p^t$.

  We have that if $T$ is a prefix of $\calT(x,y,\rho)$ then $g(x,y,\rho)\in G_T$; thus $\Pr_\rho[T \text{ is a prefix of }\calT(x,y,\rho)] \leq p_t$.

  Meanwhile, $T$ is a prefix of $\calT(x,y,\rho)$ if $g(x,y,\rho)\in G_T$ and $g(x,y,\rho)$ is complete.  
  By the inclusion-exclusion principle,
  \begin{align*}
    \Pr[T \text{ is a prefix of } \calT(x,y,\rho)] &=  \Pr[g(x,y,\rho)\in G_T] + \Pr[g(x,y,\rho) \text{ is complete}] - \\
    &\qquad\qquad\qquad\qquad \Pr[g(x,y,\rho)\in G_T \text{ or } g(x,y,\rho) \text{ is complete}]\\
    &\geq p^t + \Pr[g(x,y,\rho) \text{ is complete}] - 1
    %&\geq p^t - 1/n^2\\
  \end{align*}
  We have that $\Pr[g(x,y,\rho) \text{ is complete}] = 1 - \Pr[\tau(x,\rho) \text{ or } \tau(y,\rho) \text{ is not complete}]$. By union bound and \lemref{shorthash}, $\Pr[g(x,y,\rho) \text{ is complete}] \geq 1 - 2/n^2$.  Substituting, $\Pr[T\text{ is a prefix of }\calT(x,y,\rho)] \geq p^t - 2/n^2$.
\end{proofof}

\bigskip


\begin{proofof}{\lemref{looseupper}}
  Let $\calT$ be the set of all transformations that solve $x$ and $y$.  By 
  \lemref{hasheseqtransformation} and 
  \lemref{probinduces}, 
  \[
    \Pr_{h\in \calH} (h(x) = h(y)) = \sum_{T\in \calT} p^{|T|}.
  \]
Thus, we want to find the $\calT$ (for the given $x$ and $y$) that maximizes this probability.

  %First, note that $\calT$ must be prefix free: \todo{fill in why}.
  
  %By \lemref{prefixfree}, 
  Since all pairs $T_1, T_2\in \calT$ solve $x$ and $y$, there is no pair $T_1, T_2\in \calT$ such that $T_1$ is a prefix of $T_2$.  Thus, $\calT$ can be viewed as the leaves of a trie of branching factor at most $3$, where each leaf has depth at least $cr$.  
  
  %TODO: each non-costly edge in the trie has branching factor at most 1, so they can be collapsed; this means the cost of a leaf is exactly its depth.  
  
  %Consider a nodes of the trie at depth $cr$ (if any does not exist, we can increase the collision probability of $S$ by adding paths to these nodes in the trie).  Consider
  We show that without loss of generality all leaves are at depth $cr$.  Consider a leaf $T_1$ at the maximum depth of the trie $i > cr$, and its siblings $T_2$ and $T_3$ if they exist.  Collapse this leaf and its siblings, replacing them instead with a leaf $T_p$ corresponding to their parent in the trie; call the resulting set $\calT'$.  Since we have added a transformation of length $i-1$ and removed at most three of length $i$, this  changes the total cost of $\calT$ by at least $p^{i-1} - 3p^{i}$; this is positive since $p \leq 1/3$.
  %\begin{align*}
  %  \sum_{s\in S'} p^{\text{cost}(s)} &= \left(\sum_{s\in S} p^{\text{cost}(s)}\right) - p^{\text{cost}(s_1)} - p^{\text{cost}(s_2)} - p^{\text{cost}(s_3)} + p^{\text{cost}(s_p)}\\
  %  &\geq \sum_{s\in S} p^{\text{cost}(s)}
  %\end{align*}
Repeating this process results in a set $\calT_M$ with all nodes at depth $cr$, where $\calT_M$ gives larger collision probability than the original set $\calT$.  

  There are at most $3^{cr}$ transformations in $\calT_M$, each of length $cr$.  Thus
  \[
    \Pr_{h\in \calH} (h(x) = h(y)) \leq 3^{cr} p^{cr}.\qedhere
  \]
\end{proofof}

\bigskip

\begin{proofof}{\lemref{nomatchcollisionprob}}
  Let $\hat{x}$ and $\hat{y}$ be arbitrary $\$$-terminal strings of length $cr$ with no other characters in common.  We use grid walks on $G(\hat{x},\hat{y})$ to reason about grid walks on $G(x,y)$.

  Let $GR(i,j)$ be the set of all grid walks reaching node $(i,j)$ in $G(\hat{x},\hat{y})$.  Let $W(i,j) = \Pr[g(\hat{x},\hat{y},\rho)\in GR(i,j)]$.  We have $W(0,0) = 1$.  

  Clearly, $GR(i,j)$ is a subset of $GR(i-1,j) \cup GR(i-1,j-1) \cup GR(i,j-1)$.  In fact, using a case-by-case analysis essentially identical to that of \lemref{probinduces}, 
  \[
    W(i,j) \leq p \cdot W(i-1,j) + p\cdot W(i-1,j-1) + p\cdot W(i,j-1).
  \]
  We take $W(i^*,-1) = 0 = W(-1,j^*)$ for all $i^*$ and $j^*$ so that we can state this recursion without border cases.

  We show by induction that if $\max{i,j} = \ell$, then $W(i,j) \leq (2p/(1-p))^{\ell}$.  This is already satisfied for $\ell = 0$. 

  Assume that the induction is satisfied for all $W(i^*,j^*)$ with $\max\{i^*,j^*\} = \ell - 1$.  For all $(i,j)$ such that $\max\{i,j\} = \ell$, at most two of $(i-1,j-1)$, $(i-1,j)$, and $(i,j-1)$ have max $\ell - 1$; the remaining pair has max $\ell$.  Thus 
  \[
    W(i,j) \leq p\left(\frac{2p}{1-p}\right)^{\ell - 1} + p\left(\frac{2p}{1-p}\right)^{\ell - 1} + p\left(\frac{2p}{1-p}\right)^\ell \leq \left(\frac{2p}{1-p}\right)^{\ell}
  \]

  All grid walks in $G(x,y)$ that go through $(|x|-1,|y|-1)$ must be in $GR(|x|-1,|y|-1)$.  Since we must have $\max\{|x|,|y|\} = cr + 1$, the proof is complete.
\end{proofof}

\bigskip

\begin{proofof}{\lemref{epsilonroundedrho}}
  For simplicity, we let $\hat{p_a} = p_a + \epsilon$ and $\hat{p_r} = p_r + \epsilon$.  

  Since $p_1 = \Omega(1/(r3^r n^{1/c})$, we have (omitting constants for simplicity) $p = 1/(3n^{1/rc})$.  Therefore, $p_a = \sqrt{1/(1 + 3n^{1/rc})} \gg 1/n$, and thus $p_r = p_a/(1- p_a) \gg 1/n$.  Thus, $p_a < \hat{p_a} < p_a(1 + 1/n)$ and $p_r < \hat{p_r} < p_r(1 + 1/n)$.

  Let $\epsilon'$ satisfy
  \begin{equation}
    \eqlabel{perturbedps}
    p(1 - \epsilon') \leq \frac{\hat{p_a}(1-\hat{p_a})\hat{p_r}}{(1 - \hat{p_a}^2)} \leq p(1 + \epsilon') \qquad \text{ and } \qquad 
    p(1 - \epsilon') \leq \frac{(1-\hat{p_a})^2\hat{p_r}^2}{(1 - \hat{p_a}^2)} \leq p(1 + \epsilon').
  \end{equation}
  Then the proof of \lemref{probinduces} gives that for any $\$$-terminal strings $x$ and $y$, and any transformation $T$ of length $t$, 
  \[
    (p(1-\epsilon'))^t - 1/n^2 \leq \Pr_{\rho}[T \text{ is a prefix of }\calT(x,y,\rho)] \leq (p(1 + \epsilon'))^t.
  \]
  So long as $(1 \pm \epsilon')^t = \Theta(1)$ we are done.  Clearly this is the case for $\epsilon' = O(1/n)$ since $t \leq 2d = O(n)$.
  We prove each bound in Equation~\eqref{perturbedps} one term at a time for $\epsilon' = O(1/n)$.  

  \noindent
  First inequality (recall that $p_a \leq 1/2$): 
  \[
    \frac{\hat{p_a}(1 - \hat{p_a})\hat{p_r}}{(1 - \hat{p_a}^2)} > \frac{p_a(1 - p_a(1 + 1/n))p_r}{1 - p_a^2} = p - \frac{p_ap_r}{n(1 - p_a^2)} = p - \frac{p}{n(1 - p_a)} = p(1 - O(n))
  \]
  Second inequality: 
  \begin{align*}
    \frac{\hat{p_a}(1 - \hat{p_a})\hat{p_r}}{(1 - \hat{p_a}^2)} &< \frac{p_a(1 + 1/n)^2(1 - p_a)p_r}{1 - (p_a(1 + 1/n))^2} = \frac{p_a(1 - p_a)p_r}{1/(1 + 1/n)^2 - p_a^2} \\
    &= \frac{p_a(1 - p_a)p_r}{1 - O(1/n^2) - p_a^2} < \frac{p_a(1 - p_a)p_r}{(1 - p_a^2) (1 - O(1/n^2))} \\
    &= p(1 + O(1/n^2))
  \end{align*}
  Third inequality (since $p_a \leq 1/2$, $2p_a \leq 4(1 - p_a)^2$): 
  \begin{align*}
    \frac{(1-\hat{p_a})^2\hat{p_r}^2}{(1 - \hat{p_a}^2)} &\geq 
    \frac{(1-p_a(1 + 1/n))^2p_r^2}{(1 - {p_a}^2)} \\
    &= \frac{(1 - 2p_a(1 + 1/n) + p_a^2(1 + 1/n)^2)p_r^2}{(1 - {p_a}^2)} \\
    &> \frac{((1-p_a)^2 - 2p_a/n)p_r^2}{(1 - {p_a}^2)} = p - \frac{2p_ap_r^2}{n(1 - {p_a}^2)} \\
    &\geq p(1 - O(1/n)) 
  \end{align*}
  Fourth inequality (this is largely the same as the second inequality): 
  \begin{align*}
    \frac{(1-\hat{p_a})^2\hat{p_r}^2}{(1 - \hat{p_a}^2)} &\leq 
    \frac{(1-{p_a})^2p_r(1 + 1/n)^2}{1 - ({p_a}(1 + 1/n))^2} = p(1 + O(1/n^2))
    % \frac{(1-{p_a})^2(p_r(1 + 1/n))^2}{(1 - {p_a})^2(1 - O(1/n^2))} 
  \end{align*}
\end{proofof}


==> potential.tex <==
%old math for the potential function version

\newcommand{\cost}{\text{cost}}
\newcommand{\dist}{\text{dist}}


  \begin{lemma}
    The total cost of all paths of weight more than $2cr$ is at most 
    \[
      \left(\frac{2p}{1-p}\right)^{cr}
    \]
  \end{lemma}
  \begin{proof}
  \end{proof}

  \begin{lemma}
    We can upper bound the cost of any graph using a graph that consists of a series of levels, each of length exactly $cr$.  The cost of all nodes in the first level is $1$. 
  \end{lemma}

  \begin{proof}
    Any nodes outside the original graph only increase the cost.  We're OK to chop things off outside the main diagonal from the last lemma.  
  \end{proof}

  \begin{lemma}
    There are only $O(i^2)$ non-matching nodes at distance $i$. 
  \end{lemma}

  \begin{proof}
    Look at each $j$ on a given level.  Every time it is non-matching, its value increases by $1$.  Thus, we can only have $i$ nodes at distance $i$ for each $j$.  By definition, any node $(i,j)$ has distance at least $j$ because it is at least $j$ from the diagonal.  
  \end{proof}


Define $\cost(i,j)$ to be either the total cost of all transformations ending at $i,j$ if $x_{i-1}\neq y_{j-1}$, or $0$ otherwise. 

  Define a potential function 
  \[
    \Phi(i,j) = \frac{\cost(i,j)}{\left(\frac{2p}{1-p}\right)^{\dist(i,j)}}.
  \]

  \begin{lemma}
    The total cost of a graph is bounded by $\sum \Phi \left(\frac{2p}{1-p}\right)^{cr}$, summing over all nodes $(i,j)$ along a single level.
  \end{lemma}
  \begin{proof}
    Using the logic I had before, we only need to count the cost of all nodes of distance $cr$.  Take the one with the most cost.   
   Partition all paths into equivalence classes based on which node of cost $cr$ they go through first.  
    Paths through nodes at lower levels cannot contribute to the biggest one's cost.  All nodes at the same level as the big node CAN contribute to its cost.  They all have distance at least $cr$ (due to the partitioning); thus their cost satisfies the equation above.  The cost of all paths going through node $i$ and ending at node $j$ is at most the cost of all paths going through node $i$ (because you're just multiplying another probability).
  \end{proof}

  Let $\Phi(i)$ be the total potential of all nodes at level $i$. 

  \begin{lemma}
    For all $i$, $||\Phi(i)|| \geq ||\Phi(i+1)||$.
  \end{lemma}
  \begin{proof}
    Consider the contribution of $\Phi(i,j)$ to $\Phi(i,)$ 
  \end{proof}

  \begin{lemma}
    The total cost of level $i$ is at most $(2p/(1-p))$ times the cost of level $i-1$.
  \end{lemma}

  \begin{proof}
    Consider the contribution of node $(i-1, j)$ to level $i$.  This contribution is:
    \[
      \cost(i-1,j) \left(\sum_{k = 0}^{cr - j} 2p^{k + 1} \right) \leq \cost(i-1,j)\frac{2p}{1-p}.
    \]

    Let $(i,j)$ be a
  \end{proof}

  \begin{lemma}
    For all $i$, $\Phi(i)\geq \Phi(i+1)$.
  \end{lemma}
  \begin{proof}
    We upper bound $\Phi(i+1)$ by summing over the contribution to $\Phi(i+1)$ for each $\Phi(i,j)$.

    TODO: partition $\Phi(i+1)$ into parts depending on which node at level $i$ the cost came from.  

    If $(i,j)$ is a match, the contribution of $\Phi(i,j)$ to $\Phi(i+1)$ is $\Phi(i,j)$.  

    If $(i,j)$ is not a match, let $(i+1,j')$ be the first node below $j$ on level $i+1$ that is a match.  Then $\Phi(i+1)$ increases by
    \[
      \Phi(i,j)\left(\frac{2p}{1-p}\right)^{\dist(i,j)} \left( \sum_{k=1}^{j'-j} p^{k}/\left(\frac{2p}{1-p}\right)^{\dist(i+1,j+k)} + \sum_{k=1}^{j'-j-1} p^{k}/\left(\frac{2p}{1-p}\right)^{\dist(i+1,j+k+1)} \right)
    \]
    Assume that for all $j$, $d = \dist(i,j)$, and that for all $j$, $\dist(i+1,j)\leq d+1$.  Then we can upper bound the contribution to $\Phi(i+1)$ by 
    \begin{align*}
      \Phi(i,j)\left(\frac{2p}{1-p}\right)^{d} \left( \sum_{k=1}^{j'-j} p^{k}/\left(\frac{2p}{1-p}\right)^{d+1} + \sum_{k=1}^{j'-j-1} p^{k}/\left(\frac{2p}{1-p}\right)^{d+1} \right) \leq \\
      \Phi(i,j)/\left(\frac{2p}{1-p}\right) \left( \sum_{k = 1}^{j' - j} p^k + \sum_{k = 1}^{j' - j-1} p^k \right) \leq \Phi(i,j). 
    \end{align*}

    Otherwise, we can assume that for all $k$, $\dist(i+1,j+k) \leq \dist(i,j) + k$.  
 Then we can upper bound the contribution to $\Phi(i+1)$ by 
    \begin{align*}
      \Phi(i,j)\left(\frac{2p}{1-p}\right)^{d} \left( \sum_{k=1}^{j'-j} p^{k}/\left(\frac{2p}{1-p}\right)^{d+k} + \sum_{k=1}^{j'-j-1} p^{k}/\left(\frac{2p}{1-p}\right)^{d+k} \right) \leq \\
\Phi(i,j) \left( \sum_{k=1}^{j'-j} p^{k}/\left(\frac{2p}{1-p}\right)^{k} + \sum_{k=1}^{j'-j-1} p^{k}/\left(\frac{2p}{1-p}\right)^{k} \right)\leq \\
      2\Phi(i,j) \sum_{k=1}^{j'-j} \left(\frac{1-p}{2}\right)^k \leq 2\Phi(i,j)\frac{1 - p}{2(1 - p} \leq \Phi(i,j)\frac{2-2p}{1+p}
    \end{align*}

    Otherwise, we can assume that for all $k$, $\dist(i+1,j+k) \leq \dist(i,j) + k$.  
 Then we can upper bound the contribution to $\Phi(i+1)$ by 
    \begin{align*}
      \Phi(i,j)\frac{p}{2p/(1-p)}  + \Phi(i,j)\left(\frac{2p}{1-p}\right)^{d} \left( \sum_{k=1}^{cr - j} (1 + p)p^{k}/\left(\frac{2p}{1-p}\right)^{d+k}  \right) \leq \\
      \Phi(i,j) \left( \frac{p}{2p/(1-p)} + (1 + p)\sum_{k=1}^{cr-j} \left(\frac{1-p}{2}\right)^k  \right) \leq \\ 
      \Phi(i,j) \left( \frac{p}{2p/(1-p)} + (1 + p)\frac{1-p}{2(1 - (1-p)/2)} \right)
    \end{align*}

  \end{proof}
    

  \begin{lemma}
    Assume a graph $G'$ has no matches for the first $i-1$ levels.  Then there is a graph $G'$ with no matches for the first $i$ levels that has larger potential for all nodes for levels $i+1$ and up. 
  \end{lemma}

  \begin{proof}
    Assume that the matches of $G$ at level $i$ are at $j_1,j_2,\ldots j_k$, starting at the center and going outwards. 

      Then all nodes $j \leq j_k$ at level $i+1$ have distance $i$, and all nodes $j > j_k$ at level $i+1$ have distance $i+1$. 

      Also, we can directly calculate the cost of all nodes $j$ at level $i+1$.  If $j\leq j_k$, let $j_p$ be the match immediately before $j$.  
      \[
        \Phi(j,i+1) = \frac{\cost(j_p,i)p^{j-j_p-1} + \sum_{k=j_p+1}^{j} \cost(k,i)p^{1 + j - k}}{\left(\frac{2p}{1-p}\right)^{i}}
      \]

      Let us calculate the potential after all matches have been removed. 
      \[
        \Phi'(j,i+1) = \frac{ \sum_{k=0}^{j} \cost(k,i)p^{1 + j - k}}{\left(\frac{2p}{1-p}\right)^{i+1}}
      \]
      Taking the difference and removing positive terms,
      \[
        \Phi'(j,i+1) - \Phi(j,i+1) \geq \frac{\cost(j_p,i)\left(2p^{j-j_p+1} + p^{j-j_p} - p^{j-j_p-1}\left(\frac{2p}{1-p}\right) \right)}{(2p/(1-p))^{i+1}}
      \]

  \end{proof}

    \begin{lemma}
    Assume that any graph $G'$ has potential blah on level $i$.  Then there exists a $G''$ that also has potential blah on level $i$, has larger potential on level $i+1$, and has no matches between levels $i$ and $i+1$.  
    \end{lemma}

    \begin{proof}
      Let $(i,j)$ be the first match on level $i$, and let $(i+1,j_2)$ be the next match on level $i+1$ (i.e. $j_2$ is the smallest $j_2 > j$ such that $(i+1,j_2)$ is a match).  Then the contribution of $\Phi(i,j)$ to $\Phi(i+1)$ is at most 
      \[
        \sum_{k=j+1}^{j_2} \frac{\Phi(i,j)p^{k-j-1}}{(2p/(1-p))^{\dist(i+1,k)}}.
      \]
      Furthermore, all paths going through $\Phi(i,j)$ don't have the chance to contribute to $\Phi(i,j')$ for $j' > j$. 

      Once we remove the match, the contribution of $\Phi(i,j)$ to $\Phi(i+1)$ is at most 
      \[
        \sum_{k=j+1}^{j_2} \frac{\Phi(i,j)(p^{k-j} + p^{k-j+1})}{(2p/(1-p))^{\dist(i+1,k)}}.
      \]
      Furthermore, all paths going through $\Phi(i,j)$ now increase $\Phi(i)$ as well; this only increases $\Phi(i+1)$. 
    \end{proof}

  \begin{lemma}
    The graph satisfying the above that maximizes $\Phi(i)$ has no matches.
  \end{lemma}
  \begin{proof} 
Using the above claim, we proceed backwards through the levels of $G$.  We use the claim to remove all matches along level $i$, replacing $G$ with a graph $G'$ that is identical to $G$ for the first $i-1$ levels, has no matches on level $i$, and is entirely different from $G$ on the remaining $cr-i$ levels.  We then begin again, using the above claim to remove the matches along the last level from $G'$.

    After $2^{cr}$ iterations of the above process, we are left a graph that has no matches along any level. 
  \end{proof}

  \begin{lemma}
    The graph satisfying the above with no matches has $\Phi(i,j)\leq 1$ for all $i,j$.
  \end{lemma}
  \begin{proof}
     This is where we use the definition of $\Phi$.  This is done using an two-dimensional induction, crawling down the side of each level.  
  \end{proof}

  \begin{lemma}
    Another squared attempt
  \end{lemma}

  \begin{proof}
Let $a_{k,j} = (2/(1-p))^{k-j}(1+p)$ if $k < j$, and $a_{k,k} = p$.  
    By definition, we have
    \begin{align*}
      \Phi(i+1) &= \sum_{j = 0}^{cr} \Phi(i+1,j)^2 = \sum_{j=0}^{cr}\left(\sum_{k=0}^j \Phi(i,k) a_{k,j}\right)^2 \\
      &= \sum_{j=0}^{cr} \sum_{k=0}^{j} \Phi(i,k)^2 a_{k,j}^2 + 2\sum_{k' = k+1}^{j} \Phi(i,k)\Phi(i,k')a_{k,j}a_{k',j}\\
      &=  \sum_{k=0}^{cr} \sum_{j=k}^{cr} \Phi(i,k)^2 a_{k,j}^2 + 2\sum_{k' = k+1}^{cr} \sum_{j=k'}^{cr} \Phi(i,k)\Phi(i,k')a_{k,j}a_{k',j}\\ 
      &=  \sum_{k=0}^{cr}  \Phi(i,k)^2 \sum_{j=k}^{cr} a_{k,j}^2 + 2\sum_{k' = k+1}^{cr} \Phi(i,k)\Phi(i,k') \sum_{j=k'}^{cr} a_{k,j}a_{k',j}\\ 
      &=  \sum_{k=0}^{cr}  \Phi(i,k)^2 \left(p^2 + (1+p)^2\sum_{j' = 1}^{cr-k} \left(\frac{1-p}{2}\right)^{2j'} \right) \\
      &\qquad + 2\sum_{k' = k+1}^{cr} \Phi(i,k)\Phi(i,k') \left(p(1+p)\left(\frac{2}{1-p}\right)^{k-k'} + \left(\frac{2}{1-p}\right)^{k-k'}\sum_{j = k' + 1}^{cr} (1+p)^2 \left(\frac{2}{1-p}\right)^{2k' - 2j} \right) \\
      &\leq  \sum_{k=0}^{cr}  \Phi(i,k)^2 \left(p^2 + (1+p)^2 \frac{\left(\frac{1-p}{2}\right)^2}{1 - \left(\frac{1-p}{2}\right)^2} \right) \\
      &\qquad + 2\sum_{k' = k+1}^{cr} \Phi(i,k)\Phi(i,k') \left(\frac{2}{1-p}\right)^{k-k'} \left(p(1+p) + (1+p)^2 \sum_{j' = 1}^{cr-k'} \left(\frac{1-p}{2}\right)^{2j'} \right) \\
      &\leq  \sum_{k=0}^{cr}  \Phi(i,k)^2 \left(\frac{1 + 2p - 2p^2 + p^3}{3 - p} \right) \\
      &\qquad + 2\sum_{k' = k+1}^{cr} \Phi(i,k)\Phi(i,k') \left(\frac{2}{1-p}\right)^{k-k'} \left(p(1+p) + (1+p)^2 \frac{\left(\frac{1-p}{2}\right)^2}{1 - \left(\frac{1-p}{2}\right)^2} \right)\\
      &\leq  \sum_{k=0}^{cr}  \Phi(i,k)^2 \left(\frac{1 + 2p - 2p^2 + p^3}{3 - p} \right) + 2\sum_{k' = k+1}^{cr} \Phi(i,k)\Phi(i,k') \left(\frac{2}{1-p}\right)^{k-k'} \frac{(1 + p)^2}{3-p} \\
      &\leq  \frac{(1+p)^2}{3-p}\left(\sum_{k = 0}^{cr} \Phi(i,k) \left(\frac{2}{1-p}\right)^k  \right) \left(\sum_{k' = 0}^{cr} \Phi(i,k')  \left(\frac{2}{1-p}\right)^{-k'} \right)
    \end{align*}
  \end{proof}




==> tightupper.tex <==
In this section, we prove that for any $x$ and $y$ at distance at least $cr$, 
\[
\Pr(h(x) = h(y)) \leq (cr)^{O(1)}\left(\frac{2}{1-p}\right)^{cr}.
\]
Furthermore, we give an example $x$ and $y$ for both edit distance and Ulam distance showing that this analysis is tight up to polynomial factors in $cr$.  (These factors are lower-order terms in the final running time; see TODO.)

We regard the hash of $x$ and $y$ as the random walk of a graph $G$.  We say that the \defn{level} of a graph node is the edit distance of the corresponding substrings, and its \defn{cost} is the probability that the two substrings collide.  

We probably talk about paths through the graph, each of which correspond to an execution of the hash and also correspond to a transformation.  Each path of length $k$ occurs with probability $p^k$ (by the transformation lemma). 

\begin{lemma}
For each node $i$ at level $cr$, consider the set of all paths reaching $i$ that have not previously traversed a node at level $cr$.  

The cost of the terminal node in a graph $G$ is at most the total, over all nodes $i$ at level $cr$, of the paths reaching $i$ that have not previously reached a node at level $cr$. 
\end{lemma}

\begin{proof}
From TODO, each step in a path from a node at level $\ell$ goes to a level at most $\ell + 1$.  The terminal node is at level at least $cr$, so any path that ends in the terminal node must go through at least one node at level $cr$.  

Consider all paths first going through a node $i$ of cost $cr$.  The total probability of these paths is precisely the total probability of reaching node $i$, times the probability of reaching the terminal node from $i$.  This is less than or equal to the probability of reaching node $i$.
\end{proof}

From now on, we attempt to find the graph $G^*$ maximizing the total cost of all paths reaching nodes at level $cr$ for the first time.  

We call a level $i$ \defn{normalized} if it can be partitioned into two sets of nodes, $N_i$ and $M_i$, satisfying:
\begin{itemize}
\item If $(x,y)\in M_i$, $(x,y)$ is a match and either $(x+1,y+1)\in R_i$ or $(x+1,y+1)\in N_i$.
\item 
\end{itemize}

%even older 
\iffalse
In this section we tighten \lemref{looseupper}.  This ultimately improves the base of the exponential term in $r$ in the final running time. 

We prove our running time using the following strings:
\[
  \hat{x} = 0^{cr/2} 1^{cr/2} ~~~~~ \hat{y} = 1^{cr/2} 0^{cr/2}
\]

First, we prove that these are the worst case strings for our algorithm.
\begin{lemma}
  If $x$ and $y$ satisfy $\ED(x,y) \geq cr$, then
  \[
    \Pr_{h\in \calH} (h(x) = h(y)) \leq 
    \Pr_{h\in \calH} (h(\hat{x}) = h(\hat{y})) 
  \]
\end{lemma}

\begin{proof}
  TODO: we need to do this on the graph representation directly.  At intermediate points, we will have some graphs that are not realizeable by actual strings.  But we will end with one; namely the above.

  We first show that if $x_i = y_j$, where $i < cr/2$ or $j<cr/2$, then there exists a $x',y'$ with a larger collision probability.  

  Consider the pair $(i,j)$ with the lowest $\min\{i,j\}$ such that $x_i = y_j$; assume without loss of generality that TODO $i < j$.  There must exist a pair $(i',j')$ with $i' > i$ and $j' \geq cr/2$ such that $x_{i'} \neq y_{j'}$ (actually it's on EVERY diagonal --- so for every $i' > i$, there exists an $i'' = i' + x$ and $j'' = cr/2 + x$ such that $x_{i''} \neq y_{j''}$).  Because if not, if we consider the path from $(0,0)$ to $(i,j)$, from $(i+1,j+1)$ to $(i',cr/2)$, from $(i',cr/2)$ to $(cr/2,cr - i')$ (without cost), and finally from $(cr/2,cr - i')$ to $(cr,cr)$, we obtain total cost $cr/2 - 1 + cr/2 < cr$ at $(cr, cr)$. 

  Then, we set $(i,j)$ to no longer be a match,  and $(i'',j'')$ to be a match, where these are chosen by setting $x = 0$ (so it's $(i + 1 + x, cr/2 + x)$).

\end{proof}
   

Now, we bound the collision probabilities of these strings.
\begin{lemma}
  \lemlabel{tightupper}
  \[
    \Pr_{h\in \calH} (h(\hat{x}) = h(\hat{y})) \leq \left(\frac{2p}{1-p}\right)^{cr}
    \]
\end{lemma}
\begin{proof}
  Let $P(i,j) = \Pr_{h\in\calH} (h(0^i) = h(1^j))$.  Clearly, $P(i,j) = P(j,i)$, so
  \[
    \Pr_{h\in \calH} (h(\hat{x}) = h(\hat{y})) \leq 2 \sum_i P(i,cr/2)^2
  \]

  Consider a grid of width $i$ and height $j \geq i$.  For a path $P$, let $k$ be the number of ``right'' movements in the grid; thus $P$ has length $j +k$.  There are $\binom{j+k}{i}$ ways to choose the ``diagonal'' or ``right'' movements in the grid; then there are $\binom{i}{k}$ ways to choose the ``right'' movements among these.  Thus,
  \[
    P(i,j) = \sum_{k = 0}^i p^{j+k}\binom{j+k}{i}\binom{i}{k}.
  \]
  
  To maximize this value, we use the classic bounds (where $H(x) = -x\log_2 x - (1-x)\log_2 (1-x)$) 
  \[
    \frac{1}{n+1} 2^{n H(k/n)} \leq \binom{n}{k}\leq 2^{n H(k/n)}
  \]
  Thus,
  %\begin{align*}
    \[
    P(i,j) \leq \sum_{k = 0}^i p^{j+k} 2^{(j+k)H(i/(j+k)) + i H(k/i)}\\
  \]
       %&= i \max_k p^{j+k} 2^{(j+k)((i\log_2 (i/j+k))/(j+k) - (1 - i/(j+k))\log_2 (1 - i/(j+k))) + i( (k/i)\log_2 (i/k) - (1 - k/i)\log_2 (1 - k/i)}
  % \end{align*}
so replacing it into the above, 
  \[
    \sum_i P(i,cr/2)^2 \leq  (cr)^2\max_{i,k} p^{2(j+k)} 4^{(j+k)H(i/(j+k)) + i H(k/i)}
   \]
  Taking the log, we want to maximize 
  \begin{multline}
    (j+k) \log_2 p + (j+k)\left(\frac{i}{j+k}\log_2 \frac{j+k}{i} - \left(1 - \frac{i}{j+k}\right)\log_2 \left(1 - \frac{i}{j+k}\right)\right)\\ + k\log_2 \frac{i}{k} - i\left(1 - \frac{k}{i}\right)\log_2 \left(1 - \frac{k}{i}\right)
  \end{multline}

  To maximize over $k$, we take the derivative and set to $0$, obtaining 
  \[
  0 = \log_2 p - \log_2(1 - i/(j+k)) + \log_2(1 - k/i) + \log_2(i/k)
\]

  Thus, the minimum occurs at $p = (1 - i/(j+k))(i/k - 1)$, so 
      
    %(j+k) \log_2 p + (j+k)(\frac{i}{j+k}\log_2 \frac{j+k}{i} - (1 - \frac{i}{j+k})\log_2 (1 - \frac{i}{j+k}))\\ + k\log_2 \frac{i}{k} - i(1 - \frac{k}{i})\log_2 (1 - \frac{k}{i})
\end{proof}

\fi


\iffalse 
  \begin{lemma}
    OLD PROOF
  \end{lemma}
\begin{proof}
  Let 
  \[
    \Phi(i,j) = \frac{\cost(i,j)}{\left(\frac{2p}{1-p}\right)^{\dist(i,j)}}.
  \]

  Let the set of distances in one column be $d_1,\ldots, d_{cr}$, and in the next be $d_1',\ldots, d_{cr}'$.  

  By definition,
  \[
    \sum_{j = 0}^{cr} \Phi(i+1,j) \left(\frac{2p}{1-p}\right)^{d_j'} = p\sum_{j=0}^{cr} \Phi(i,j) \left(\frac{2p}{1-p}\right)^{d_j} + \Phi(i,j-1) \left(\frac{2p}{1-p}\right)^{d_{j-1}} + \Phi(i+1,j-1) \left(\frac{2p}{1-p}\right)^{d_{j-1}'}
  \]
  \[
    \sum_{j = 0}^{cr} \Phi(i+1,j) \left(\frac{2p}{1-p}\right)^{d_j'}- p\Phi(i+1,j-1) \left(\frac{2p}{1-p}\right)^{d_{j-1}'} = p\sum_{j=0}^{cr} \Phi(i,j) \left(\frac{2p}{1-p}\right)^{d_j} + \Phi(i,j-1) \left(\frac{2p}{1-p}\right)^{d_{j-1}} 
  \]
  \[
    \sum_{j = 0}^{cr} \Phi(i+1,j) - p\Phi(i+1,j-1) \left(\frac{2p}{1-p}\right)^{d_{j-1}'-d_j'} = p\sum_{j=0}^{cr} \Phi(i,j) \left(\frac{2p}{1-p}\right)^{d_j-d_j'} + \Phi(i,j-1) \left(\frac{2p}{1-p}\right)^{d_{j-1}-d_j'} 
  \]
  \[
    \sum_{j = 0}^{cr} \Phi(i+1,j)\left(1 - p\left(\frac{2p}{1-p}\right)^{d_{j}'-d_{j+1}'}\right) = p\sum_{j=0}^{cr} \Phi(i,j)\left( \left(\frac{2p}{1-p}\right)^{d_j-d_j'} + \left(\frac{2p}{1-p}\right)^{d_{j}-d_{j+1}'} \right)
  \]

  We want to minimize $d_j - d_j'$, $d_j - d_{j+1}'$, and $d_j' - d_{j+1}'$ in order to maximize a given $\Phi(i+1,j)$. 

  We have $d_j' \leq d_j + 1$, $d_j' \leq d_{j-1}' + 1$, and $d_j' \leq d_{j-1} + 1$, so $d_j' - d_j \leq 1$, $d_j' - d_{j-1}' \leq 1$, and $d_j' - d_{j-1} \leq 1$.  However, if two of these are 1, then the last one is 0.  Let $a_j$, $b_j$, and $c_j$ be binary variables with exactly two equal to $1$.  Then we have 
  \[
    \sum_{j = 0}^{cr} \Phi(i+1,j)\left(1 - p\left(\frac{2p}{1-p}\right)^{-a_i}\right) = p\sum_{j=0}^{cr} \Phi(i,j)\left( \left(\frac{2p}{1-p}\right)^{-b_i} + \left(\frac{2p}{1-p}\right)^{-c_i} \right)
  \]

  Assume that $\Phi(i+1,j)\geq\Phi(i,j)$ (clearly this is attainable if $a_i=0$, $b_i = 1$, $c_i = 1$).  Then we want to have $a_i = 0$ for all $i$.   Thus
  \[
    \Phi(i+1)(1 - p) \leq 2p\Phi(i) \left( \frac{1-p}{2p}\right).
  \]
\end{proof}
\fi


==> ulam.tex <==
\section{Ulam Metric}

In this section, we show that our algorithm achieves running time $O(dn^{1/c} + d3^r)$ in the Ulam metric.

\begin{lemma}
Consider a string $x$ where all characters in $x$ are unique, and $y = \pi(x)$ for some permutation $\pi$.  Then if $\Ulam(x,y) \geq cr$,
\[
\Pr_{h\in\calH_p} \left(h(x) = h(y)\right) \leq cr p^{cr}
\]
\end{lemma}

